Joint Chance Constrained Optimal Control via Linear Programming

We establish a linear programming formulation for the solution of joint chance constrained optimal control problems over finite time horizons. The joint chance constraint may represent an invariance, reachability or reach-avoid specification that the trajectory must satisfy with a predefined probability. For finite state and action spaces, the solution is exact and our method computationally superior to approaches in the literature. For continuous state or action spaces, our linear programming formulation enables basis function approximations.

==> sections/ApproximationsForContSpaces.tex <==


\section{Approximations for Continuous Spaces}
\label{sec_approx_for_cont}
Recall that the constraints in LP \eqref{eq_lp_ccoc} must hold over all states and inputs; infinitely many if the state and input spaces are continuous. In such cases approximations have to be introduced, e.g., via gridding or basis functions. Therefore, in the following we impose the state space $\Tilde{\mathcal{X}}$ to be compact.

\subsection{Gridding}
Let there be a finite partitioning of the state and input space into $\Tilde{\mathcal{X}} = \cup_{j=1}^{M_x}\Tilde{\mathcal{X}}_j$ and $\mathcal{U}=\cup_{j=1}^{M_u}\mathcal{U}_j$, where each set $\Tilde{\mathcal{X}}_j$ has non-zero $\nu$-measure, $M_x, M_u \in\mathbb{N}$. The sets $\Tilde{\mathcal{X}}_j$ are chosen such that they do not contain states with differing values for the augmented states and the MDP state components are fully contained in either $\mathcal{A},\mathcal{T}$ or $\mathcal{X}\setminus(\mathcal{A}\cup \mathcal{T})$. Let $\{\Tilde{s}_j\in\Tilde{\mathcal{X}}_j\}_{j=1}^{M_x}$ and $\{a_j\in\mathcal{U}_j\}_{j=1}^{M_u}$ be arbitrary points of these sets and the grid size of the discretization be defined as $\Delta = \max_{1\leq j \leq M_x}\sup_{\Tilde{x}_1,\Tilde{x}_2\in \Tilde{\mathcal{X}}_j}||\text{proj}_{\mathcal{X}}(\Tilde{x}_1-\Tilde{x}_2)||_2$, where $\text{proj}_{\mathcal{X}}(\cdot)$ denotes the projection onto the space $\mathcal{X}$. %and $\delta_u = \max_{1\leq j \leq M_u}\sup_{u_1,u_2\in \mathcal{U}_j}||x_1-x_2||_2$. 
For the resulting finite MDP the LP \eqref{eq_lp_ccoc} reads as
\begin{equation}
    \begin{split}
        \max_{\substack{ \lambda\in\mathbb{R}_{\geq 0},\\J_{0:N}\in \mathbb{R}^{M_x} }} \quad  &J_{0,l}
        \\ \text{s.t.} \quad &J_{N,j}\leq\ell_N(\Tilde{s}_j)  +\lambda(\alpha-\delta(b_j)), \\
        &J_{k,j}\leq  \ell_k(\Tilde{s}_j,a_i) +\hspace{-1em} \sum_{1\leq j' \leq M_x}\hspace{-1em}J_{k+1,j'}\Tilde{T}(\Tilde{X}_{j'}|\Tilde{s}_j,a_i),
    \end{split}
    \label{eq_lp_ccoc_discrete}
\end{equation}
where $b_j$ is the augmented state of $\Tilde{s}_j$, $l\in[0,M_x]$ is the index of the set $\Tilde{\mathcal{X}}_l$, which contains the initial state $\Tilde{x}_0$, $J_{k,j}$ denotes the $j$'th entry of the vector $J_k$ and the constraints hold for all $1\leq j \leq M_x$, $1\leq i \leq M_u$. The discrete version of the LP \eqref{eq_lp_ccoc_value_functions} follows accordingly. The optimal mixed policy for the discretized version of Problem \eqref{eq_problemFormulation_CCOC} is constructed by mixing the cheapest and safest greedy policies on the resulting value functions. %The set of optimal inputs at a given state and time step is easily identified by the set of active constraints of the LP \eqref{eq_lp_ccoc_discrete}. 
Under the mixing ratios in \eqref{eq_stochastic_policies_ratios}, the mixed policy yields a safety of $\alpha$ when applied to the discretized dynamics. However, when applied to the continuous dynamics, the safety of the policy potentially deteriorates. Furthermore, the extent of deterioration is computationally hard to determine. Instead, we provide bounds on the difference of safety between the discretized and continuous dynamics in the following. When faced with continuous dynamics, the policy obtained for the discretized dynamics is implemented such that, if the continuous state $\Tilde{x}_k\in \Tilde{\mathcal{X}}_j, 1\leq j \leq M_x$, the action advertised for the state $\Tilde{s}_j$ is applied to the system. 
% \begin{assumption}
%     \begin{align*}
%         |t(x_{k+1}|x_k,u_k) - t(x_{k+1}|x_k,u_k')|\leq h_u||u-u'|| 
%     \end{align*} for all $x_{k+1},x_k\in\mathcal{X}, u_k,u_k'\in \mathcal{U}$.
% \end{assumption}
% \begin{proposition}
%     Let the MDP be finite, $\hat{J}_{0:N}^{\text{LP}}$ be the optimal solution of \eqref{eq_lp_ccoc_value_functions} under the optimal $\lambda$ in \eqref{eq_lp_ccoc}. Let  $\hat{J}_{0:N}^{\star}$ be the value functions associated to the optimal policy of Problem \eqref{eq_dual_of_CCOC}. Then, $\hat{J}_{0:N}^{\text{LP}}=\hat{J}_{0:N}^{\star}$. Further, the greedy policy on $\hat{J}_{0:N}^{\text{LP}}$ coincides with the state-input pairs that form active constraints in the LP \eqref{eq_lp_ccoc_value_functions}.
% \end{proposition}
% \begin{proof}
%     The equivalence of $\hat{J}_{0:N}^{\text{LP}}=\hat{J}_{0:N}^{\star}$ is a direct consequence of tdoref, since any representative point $x_j$ is associated non-zero $v$-measure.

    
% \end{proof}
% Above Proposition is useful in two ways. Firstly, it allows to characterize the optimal policies by the active constraints of the LP. Using the recursions tdoref and tdoref and restricting to inputs that form active constraints at the given state, we can solve for the cheapest and safest $\lambda^{\star}$-optimal policies $\pi_c$ and $\pi_v$. Note that the analysis in \cite{schmid2023Jccoc}, which holds for finite as well as continuous systems. Hence, if Problem \eqref{eq_problemFormulation_CCOC} is feasible for the discretized dynamics, the policy $\pi_v$ will have a safety of at least $\alpha$. Let the associated safety and costs in the discretized formulation, computed using recurions tdoref and tdoref, be $\hat{V}_{\pi_c}$, $\hat{V}_{\pi_v}$, $\hat{C}_{\pi_c}$ and $\hat{C}_{\pi_v}$, respectively. Let the policies be mixed according to 
% \begin{align}
% \label{eq_stochastic_policies_ratios}
% \pi_{\text{mix}}=\begin{cases}
% \pi_{\overline{\lambda}} & \text{with probability } p_{\overline{\lambda}}\!=\!\frac{\alpha - V_0^{\pi_{\underline{\lambda}}}(\Tilde{x}_0)}{V_0^{\pi_{\overline{\lambda}}}(\Tilde{x}_0) - V_0^{\pi_{\underline{\lambda}}}(\Tilde{x}_0)}, \\
% \pi_{\underline{\lambda}} & \, \text{otherwise.}
% \end{cases}
% \end{align}
% Then, under the discretized dynamics, the mixed policy solves Problem \eqref{eq_problemFormulation_CCOC} to optimality \cite{schmid2023Jccoc}. 


%This is easily obtained from the safety of its constructing policies which has been computed via recursion tdoref to solve for the optimal mixing probabilities. Let the safety of the mixed policy, when applied to the continuous system, be denoted by $V_{\pi_{\text{mix}}}$, which is usually hard to compute in practice. 
\begin{assumption}
    The transition kernel $T$ admits a Lipschitz continuous density $t$, \begin{align*}
        |t(x_{k+1}|x_k,u_k) - t(x_{k+1}|x_k',u_k)|\leq h_x||x_k-x_k'||, 
    \end{align*} for all $x_{k+1},x_k,x_k'\in\mathcal{X}, u_k\in \mathcal{U}$.
    \label{ass_lipschitz_cont}
\end{assumption}
\begin{proposition}
    Let the safety of the mixed policy $\pi_{\text{mix}}$ at the initial state $x_0$ when applied to the continuous dynamics be denoted by $\hat{v}_{\pi_{\text{mix}}}$, and when applied to the discretized dynamics be denoted by $v_{\pi_{\text{mix}}}$. Under Assumption \ref{ass_lipschitz_cont}, the safety of $\pi_{\text{mix}}$ applied to the continuous system is bounded by $||\hat{v}_{\pi_{\text{mix}}}-v_{\pi_{\text{mix}}}||\leq N\gamma h_x\Delta$, where $\gamma$ is the Lebesgue measure of the set $\mathcal{A}$ for invariance and reach-avoid specifications and $\mathcal{X}\setminus\mathcal{T}$ for reachability specifications.
\end{proposition}
\begin{proof}
    Let the safety of the cheapest and safest $\lambda^{\star}$-optimal policy when evaluated on the discretized dynamics by denoted by $v_{c}$ and $v_{v}$, and when applied to the continuous system be denoted by $\hat{v}_{c},\hat{v}_{v}$, respectively. We know that $||\hat{v}_{c}-v_{c}||\leq N\gamma h_x\Delta$ and $||\hat{v}_{v}-v_{v}||\leq N\gamma h_x\Delta$ by \cite{abate2010approximate}. Hence, for any mixed policy, which has safeties $p_{v}v_{v} + (1-p_{v})v_{c}$ when evaluated on the discretized dynamics and $p_{v}\hat{v}_{v} + (1-p_{v})\hat{v}_{c}$ when applied to the continuous dynamics, respectively, we obtain 
    \begin{align*}
        ||\hat{v}_{\text{mix}}\!-\!v_{\text{mix}}||\!
        &=\!||p_{v}\hat{v}_{v}\!+\!(1\!-\!p_{v})\hat{v}_{c}\!-\!p_{v}v_{v}\!-\!(1\!-\!p_{v})v_{c}||\\
        &\leq\!||p_{v}(\hat{v}_{v}\!-\!v_{v})||\!+\!||(1\!-\!p_{v})(\hat{v}_{c}\!-\!v_{c})||\\
        &\leq\!|p_{v}|N\gamma h_x\Delta\!+\!|(1\!-\!p_{v})|N\gamma h_x\Delta\\
        &=\!N\gamma h_x\Delta.
    \end{align*}
\end{proof}
Since this bound can be computed a-priori, the safety level $\alpha$ can be tightened accordingly to guarantee a desired safety probability despite errors introduced by gridding.



% \begin{proposition}
%     Let $\lambda^{\star}$ be zero. Taking the safest $\lambda^{\star}$-optimal policy is an optimal solution. Let $\lambda^{\star}$ be equal to one, then the cheapest $\lambda^{\star}$-optimal policy is the optimal solution if it has safety greater $\alpha$. If not, the problem is infeasible. Let $\lambda^{\star}\in(0,1)$. The mixed policy tdoref is the optimal solution to the discrete LP.
% \end{proposition}
% \begin{proof}
%     First two cases are trivial. Third case:
%     The space of lambda optimal policies forms a single point or a continuous line (since it is convex) in the performance set. Taking the cheapest and the safest policy among the lambda optimal policies we can obtain the performances of all policies on the line by interpolation. Since $\lambda^{\star}$ is optimal, the optimal mixed policy is on that line and has safety $\alpha$. Hence, we can construct it by interpolating as in eq. tdoref.
% \end{proof}
%and $\pi_c$ and $\pi_v$ the associated minimum cost and maximum secondary policy. 

\subsection{Basis Function Approximations}
An alternative approach lies in approximating the value functions using basis functions, i.e., $J_{k}(\Tilde{x}_k)=\sum_{i=0}^{M-1}\beta_i\phi_i(\Tilde{x}_k)$, with parameters $\beta_i\in\mathbb{R},i\in[M-1]$ and basis functions $\phi_i:\Tilde{\mathcal{X}}\rightarrow\mathbb{R}$ \cite{defarias2003linear, mohajerin2018infinite, schmid2022probabilistic}. The $M$ basis functions are chosen a-priori and the LP optimizes over the parameters $\beta_i$. Due to approximation errors and computational aspects, it is not meaningful to compute the safest and cheapest greedy policies on the value functions obtained by LP \eqref{eq_lp_ccoc_value_functions}. Instead, one might directly apply any greedy policy associated to the results of LP \eqref{eq_lp_ccoc_value_functions} under an optimal $\lambda$ of LP \eqref{eq_lp_ccoc}, yielding the method a heuristic without explicit guarantees but with potentially better scalability than gridding. 

%We further aim to solve Problem \eqref{eq_dual_of_CCOC} under basis-function approximations of the value functions $J_{k}(x_k)=\sum_{i=M}\beta_i\phi_i(x_k)$, with parameters $\beta\in\mathbb{R}$ and basis functions $\phi_i:\mathcal{X}\rightarrow\mathbb{R}$ \cite{defarias2003linear}. The $M$ basis functions are chosen a-priori and the LP optimizes over the parameters $\beta_i,i\in[M]$. Under this approximation method, it is not practically meaningful to compute the safest and cheapest policy within the $\lambda^{\star}$ optimal policies due to approximation errors incurred by this method. Instead we directly apply the greedy policy associated to the results of Problem \eqref{eq_lp_ccoc_value_functions} under an optimal $\lambda$ of Problem \eqref{eq_lp_ccoc}. We do not provide conditions that guarantee optimality of the method, leaving basis function approximations as a useful heuristic without guarantees. We analyse the performance of the approach numerically instead.

==> sections/abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
We establish a linear programming formulation for the solution of joint chance constrained optimal control problems over finite time horizons. The joint chance constraint may represent an invariance, reachability or reach-avoid specification that the trajectory must satisfy with a predefined probability. Compared to the existing literature, the formulation is computationally tractable and the solution exact. %When faced with continuous state and action spaces, approximations via discretization or basis functions need to be applied. We provide explicit error bounds on the former. 
%In the case of continuous state and action spaces the linear program becomes infinite-dimensional and approximations need to be introduced. We consider gridding, for which we provide explicit error bounds, and basis-function approximations, which yield a useful heuristic with better scalability with respect to the state and input dimensionality. 
\end{abstract}

==> sections/acronym.tex <==
\begin{acronym}
\acro{ADP}{Approximate Dynamic Programming}
\acroindefinite{ADP}{an}{a}

\acro{BSA}{Basic Semialgebraic}

\acro{LP}{Linear Program}
\acroindefinite{LP}{an}{a}
\end{acronym}

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We presented a linear programming based framework to solve joint chance constrained optimal control problems, where the joint chance constraint represents either an invariance, reachability or reach-avoid specification. %For continuous state and actions spaces, gridding and basis function approximations have been discussed, where error bounds have been derived for the former. 
%In future work, we will extend the presented framework to multiple joint chance constraints and more general PCTL specifications, and explore practical applications for our methods.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Most system dynamics are non-deterministic, either naturally or due to unobservable modes, e.g., wind affecting a quadcopter \cite{schmid2022real} or biological variability \cite{pitchford2007uncertainty}. While control problems often feature a ``real" control cost objective, e.g., energy consumption or negative financial profit, additional objectives often need to be included, such as reaching or remaining in a set of states, e.g., for safety. Such behaviours can implicitly be imposed in optimal control problems by manually shaping the cost associated to individual states until the policy behaves as desired. However, without any instructive procedure it is generally hard achieve clear trade-offs between safety guarantees and the control cost \cite{Ono_2}. %The control-engineer needs a clear method to trade off safety vs. cost without requiring deep expertise or extensive finetuning of parameters.

The task of remaining in a safe set is called \textit{invariance}, that of reaching a target set \textit{reachability}, while \textit{reach-avoidance} combines both objectives. The goal of finding a policy that yields an optimal trade-off between the control cost incurred by the system and the probability of achieving one of the above specifications is described by the so called joint-chance constrained optimal control problem (cf. \cite{schmid2023Jccoc}). While this class of problems is very popular, existing solution approaches are computationally challenging (cf. \cite{Wang}). To overcome these computational issues, the state-of-the-art is to utilize approximations based on conservative bounds \cite{Ono_2, paulson, patil_1} or approximate the stochastic elements via sampling \cite{thorpe_1
%, raghuraman
, bavdekar, fochesato2022data}. Recently, \cite{schmid2023Jccoc} proposed a novel, numerically tractable Dynamic Programming (DP) algorithm that allows to determine optimal trade-offs between control cost and invariance probabilities. Moreover, the suboptimality of the solution decreases exponentially with the number of algorithm iterations. In this paper we extend this framework in the following directions: 
\begin{itemize}
    \item we include reachability and reach-avoid specifications;
    \item we compute policies using a one-shot linear programming (LP) approach with no residual suboptimality.
%    \item we provide error bounds for the optimal policy when continuous state and action spaces are discretized. 
%an instructive discussion to manage problems with continuous state and action spaces, where approximations are required. We present error bounds under gridding. Further, as a useful heuristic, our linear programming formulation allows the use of basis function approximations (approximate dynamic programming), which provides a superior scalability with the dimensionality of the state and action space over gridding. 
\end{itemize}

%It is the aim of this paper to design in particular such algorithms, that can optimally trade off the probability of satisfying a reachability, invariance, or reach-avoid specification, against increase of costs. 

%Section \ref{sec_problem} formally introduces the joint chance constrained optimal control problem. Section \ref{sec_prelim} introduces tools used by current DP-based approaches (Section \ref{sec_jcc_dp}) and our LP-based approach (Section \ref{sec_jcc_lp}) to solve such types of problems. Approximations for systems with continuous state and action spaces are discussed in Section \ref{sec_approx_for_cont} and numerically  evaluated in Section \ref{sec_examples}. We conclude with Section \ref{sec:conclusion}.


==> sections/lp_formulation.tex <==
\section{Joint Chance Constrained Dynamic Programming}
\label{sec_jcc_dp}
We aim to solve Problem \eqref{eq_problemFormulation_CCOC} using its Lagrange-Dual
\begin{equation}\label{eq_dual_of_CCOC}
    \begin{split}
        \sup_{\lambda\in\mathbb{R}_{\geq 0}}\inf_{\pi \in \Pi_{\text{mix}}} \quad  &\mathbb{E}_{x_0}^\pi\left[ \ell_N(x_N) + \sum_{k=0}^{N-1} \ell_k(x_k,u_k) \right] \\ &+ \lambda(\alpha-\mathbb{P}_{x_0}^\pi(x_{0:N}\in \mathcal{H})).
    \end{split}
\end{equation}
However, the inner infimum is intractable due to the non-Markovian structure imposed by the constraint \cite{schmid2023Jccoc}. 

\subsection{Auxiliary State Augmentation}
Recall that, by definition, $\mathcal{A}\cap\mathcal{T}=\varnothing$. For invariance specifications, we define a binary state $b_{\text{I},k}$, with $b_{\text{I},0} = \mathbb{1}_{\mathcal{A}}(x_0)$ and dynamics $b_{\text{I},k+1}=\mathbb{1}_{\mathcal{A}}(x_{k+1})b_{\text{I},k}$. Then, $\prod_{k=0}^N\mathbb{1}_{\mathcal{A}}(x_k) = b_{\text{I},N}$. Similarly, for reachability specifications we define $b_{\text{R},k}$, with $b_{\text{R},0} = \mathbb{1}_{\mathcal{T}}(x_0)$ and $b_{\text{R},k+1}=\mathbb{1}_{\mathcal{T}}(x_k) + \mathbb{1}_{\mathcal{T}^c}(x_k)b_{\text{R},k}$. Finally, for reach-avoid specifications we define the variable $b_{\text{RA},k}\in\{0,1,2\}$, with $b_{\text{RA},0} = \mathbb{1}_{\mathcal{A}}(x_0) + 2\mathbb{1}_{\mathcal{T}}(x_0)$ and 
%\vspace{-.6cm}
\begin{align*}
    b_{\text{RA},k+1} = \begin{cases}
    2, & \text{if } b_{\text{RA},k}=2 \lor  (b_{\text{RA},k}=1 \ \land \ x_{k+1}\in\mathcal{T}),\\
    1, & \text{if } b_{\text{RA},k}=1 \land  x_{k+1}\in\mathcal{A}, \\
    0, & \text{otherwise.} %b_{\text{RA},k}=0 \lor (b_{\text{RA},k}=1 \land x_{k+1}\notin(\mathcal{A}\cup\mathcal{T})) 
    \end{cases}
\end{align*}

The dynamics are illustrated in Figure \ref{fig_binary_dynamics}.
\begin{figure}[!tbp]
    \centering
    \begin{tikzpicture}
        \node[state] (q1) {$b_{k}=1$};
        \node[state, right of=q1] (q2) {$b_k=0$};
        \draw (q1) edge[loop above] node{$x_{k+1}\in\mathcal{A}$} (q1)
        (q2) edge[loop above] node{} (q2)
        (q1) edge[bend left, above] node{$x_{k+1}\notin\mathcal{A}$} (q2);
        
        \node[state, right of=q2] (q3) {$b_k=0$};
        \node[state, right of=q3] (q4) {$b_k=1$};
        \draw (q3) edge[loop above] node{$x_{k+1}\notin\mathcal{T}$} (q3)
        (q4) edge[loop above] node{} (q4)
        (q3) edge[bend left, above] node{$x_{k+1}\in\mathcal{T}$} (q4);
        
        \node[state](q5) at (3.25,-2.25)  {$b_k=1$};% (q5) {$b_k=1$};
        \node[state,left of=q5] (q6)  {$b_k=0$};
        \node[state,right of=q5] (q7)  {$b_k=2$};
        \draw (q5) edge[loop above] node{$x_{k+1}\in\mathcal{A}$} (q5)
        (q6) edge[loop above] node{} (q6)
        (q7) edge[loop above] node{} (q7)
        (q5) edge[bend left=40, below] node{$x_{k+1}\notin\mathcal{A}\cup\mathcal{T}$} (q6)
        (q5) edge[bend right=40, below] node{$x_{k+1}\in\mathcal{T}$} (q7);
        % Reach-Avoid
    \end{tikzpicture}
    \caption{Augumented state dynamics for invariance (top left), reachability (top right), and reach-avoid objectives (bottom). The arrows denote transitions of the binary state under the annotated condition. If arrows have no annotation, then the transition occurs under any condition.}
    \label{fig_binary_dynamics}
\end{figure}

\begin{lemma}
    The auxiliary state trajectories are such that
    \begin{align*}
        b_{\text{I},N}=1 &\Leftrightarrow x_{0:N}\in\mathcal{H}_{\text{I}}, \\
        b_{\text{R},N}=1 &\Leftrightarrow x_{0:N}\in\mathcal{H}_{\text{R}}, \\
        b_{\text{RA},N}=2 &\Leftrightarrow x_{0:N}\in\mathcal{H}_{\text{RA}}.
    \end{align*}
\end{lemma}
\begin{proof}
    To show the first equivalence, note that if there exists $k\in[N]$ such that $ x_k\notin\mathcal{A}$, then $b_{\text{I},k}=0$. By the stated dynamics, if $b_{\text{I},k}=0$, then $b_{\text{I},k+1}=0$, hence $b_{\text{I},N}=0$ by induction. Hence, if $b_{\text{I},N}=1$, then there does not exist $k\in[N]$ such that $x_k\notin\mathcal{A}$, hence $x_{0:N}\in\mathcal{H}_{\text{I}}$. Vice versa, if $x_{0:N}\in\mathcal{A}$, then $b_{\text{I},0}=1$ by $x_0\in\mathcal{A}$. Given $x_k\in\mathcal{A}$, $b_{\text{I},k}=1$, then $b_{\text{I},k+1}=1$; consequently $b_{\text{I},N}=1$ by induction. The proofs for the other cases follow similar arguments and are omitted in the interest of space. 
\end{proof}



We augment the system dynamics by appending the auxiliary state to capture the success in the safety specifications over the trajectory. To simplify notation we drop the index I, R and RA from the variable $b_k$ in the sequel. Depending on the specification type, we define $
\Tilde{\mathcal{X}}= \mathcal{X}\times\{0,1\}$, or $
\Tilde{\mathcal{X}}= \mathcal{X}\times\{0,1,2\}$, and $\Tilde{x}_k = (x_k, b_k)\in\Tilde{\mathcal{X}}$. The combined dynamics of the MDP and auxiliary state are described by the stochastic kernels $\Tilde{T}_{\text{I}},\Tilde{T}_{\text{R}},\Tilde{T}_{\text{RA}}:\mathcal{B}(\Tilde{\mathcal{X}})\times\Tilde{\mathcal{X}}\times\mathcal{U}\rightarrow[0,1]$, with density
\begin{align*}
    &\Tilde{t}_{\text{I}}(\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) \\&\!=\!\begin{cases}
    t(x_{k+1}|x_k,\!u_k)\!& \text{if} \ (b_{k}\!=\!0 \land b_{k+1}\!=\!0) \\& \ \ \ \lor \  (b_{k}=1 \land b_{k+1}\!=\!\mathbb{1}_{\mathcal{A}}(x_{k+1})) \\
    0 & \text{otherwise}, 
\end{cases}
\end{align*}
\begin{align*}
&\Tilde{t}_{\text{R}}(\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) \\&= \begin{cases}
    t(x_{k+1}|x_k,u_k) & \text{if} \ (b_{k}=1 \land b_{k+1}=1) \\& \ \ \ \lor \ (b_k=0 \land b_{k+1}=\mathbb{1}_{\mathcal{T}}(x_{k+1})) \\
    0 & \text{otherwise},
\end{cases}\\
&\Tilde{t}_{\text{RA}}(\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) \\&= \begin{cases}
    t(x_{k+1}|x_k,u_k) & \text{if} \ (b_{k}=2 \land b_{k+1}=2) \ \lor (b_k=1 \\ &  \ \ \ \land   \ b_{k+1}\!=\!\mathbb{1}_{\mathcal{A}}(x_{k+1})\!+\!2\mathbb{1}_{\mathcal{T}}(x_{k+1})) \\ & \ \ \ \lor \  (b_k=0 \land b_{k+1}=0) \\
    0 & \text{otherwise},
\end{cases}
\end{align*}
respectively, where $t$ is the density of $T$ and $\Tilde{x}_k = (x_k, b_k)$. Above dynamics implicitly comprise two steps. Firstly, the state component $x_k$ transitions to a state $x_{k+1}$ as described by $t$. Secondly, $b_{k+1}$ is deterministically computed based on $x_{k+1}$ and $b_k$. Combined, the density remains unchanged for combinations of $x_{k+1}$, $b_{k+1}$ and $b_k$ that are in accordance with the auxiliary state dynamics, and is set to zero otherwise. 

We overload the cost functions $l_k(\Tilde{x}_k,u_k)=l_k(x_k,u_k),\:l_N(\Tilde{x}_N)=l_N(x_N), k\in[N-1]$. Lastly, we define success indicator functions
\begin{align*}
    \delta_{\text{I}}(b_N)\!=\!\delta_{\text{R}}(b_N)\!=\!\begin{cases}
    1 &\hspace{-0.3em}\text{if }b_N\!=\!1,\\ 
    0 &\hspace{-0.3em}\text{else, }
\end{cases} \  \delta_{\text{RA}}(b_N)\!=\!\begin{cases}
    1 &\hspace{-0.3em}\text{if }b_N\!=\!2,\\ 
    0 &\hspace{-0.3em}\text{else.}
\end{cases}
%\intertext{and for reach-avoid specifications}
% \delta_{\text{RA}}(b_k)=\begin{cases}
%     1 & \text{if }b_k=2\\ 
%     0 &  \text{else. }
% \end{cases}
\end{align*} 
For generality, we again drop the index from $\delta$ and $\Tilde{T}$ in the following and say that the trajectory is safe if $\delta(b_N)=1$. This allows to express the probability of safety by the expected value of the success indicator function, i.e., $\mathbb{P}_{x_0}^\pi(x_{0:N}\in \mathcal{H})=\mathbb{E}_{x_0}^\pi\left[\delta(b_N)\right]$; hence, we can rewrite Problem \eqref{eq_dual_of_CCOC} as
\begin{equation}\label{eq_dual_with_binary}
    \begin{split}
        \hspace{-0.25em}\sup_{\lambda\in\mathbb{R}_{\geq 0}}\hspace{-1.25em}\inf_{\ \ \  \pi \in \Pi_{\text{mix}}} \hspace{-0.85em}\mathbb{E}_{\Tilde{x}_0}^\pi\hspace{-0.45em}\left[\!\ell_N(\Tilde{x}_N)\!+\hspace{-0.5em}\sum_{k=0}^{N-1} \hspace{-0.2em}\ell_k(\Tilde{x}_k,u_k)\!+\!\lambda(\alpha\!-\!\delta(b_N))\!\right]
    \end{split}.
\end{equation}
Note that this problem formulation matches with \cite{schmid2023Jccoc}, replacing $b_N$ with $\delta(b_N)$. In the sequel we extend the results in \cite{schmid2023Jccoc}. % allowing us to conclude the upcoming results. {\color{red} I feel the following paragraph is not very clear (i.e., the link) The subsequent assumption is imposed in the following.
% \begin{assumption}
%     There exists a feasible finite cost policy for Problem \eqref{eq_problemFormulation_CCOC}.
%     \label{ass_existence_of_finite_cost_feasible_policy}
% \end{assumption}
%Assumption \ref{ass_existence_of_finite_cost_feasible_policy} is needed to guarantee that the optimal $\lambda$ in  Problem \eqref{eq_dual_with_binary} is finite. 
\begin{theorem}
    The supremum and infimum in Problem \eqref{eq_dual_with_binary} are attained by some finite $\lambda \in \mathbb{R}_{\geq 0}$ and a mixed policy, respectively. The inner infimum in Problem \eqref{eq_dual_with_binary} is Lipschitz-continuous in $\lambda$. 
    \label{cor_max_min_attainable}
\end{theorem}
\ifArxivVersion
    \begin{proof}
        Given any fixed $\lambda\in\mathbb{R}_{\geq 0}$, the existence of an optimal policy for the inner infimum is guaranteed under Assumption \ref{assumption_of_attainability} \cite{schmid2023Jccoc}. Moreover, at least one such optimal policy is deterministic Markov \cite{schmid2023Jccoc}. This allows us to write $\min$ instead of $\inf$ in \eqref{eq_dual_with_binary} and restrict to the class $\Pi$ without the loss of optimality.
        
        Given the existence of a feasible finite cost policy (Assumption \ref{assumption_of_attainability}), an upper bound $\overline{\lambda}$ on $\lambda$ can be found \cite{schmid2023Jccoc}. Further, the function  $
            f(\lambda)\!=\!\min_{\pi \in \Pi}\mathbb{E}_{\Tilde{x}_0}^\pi\!\left[ \ell_N(\Tilde{x}_N)\!+\hspace{-0.4em}\sum_{k=0}^{N-1} \hspace{-0.2em}\ell_k(\Tilde{x}_k,u_k)\!+\!\lambda(\alpha\!-\!\delta(b_N))\right]$
            %\label{eq_proof_dual_problem_as_function_f_of_lambda}
        is Lipschitz-continuous in $\lambda$. To show this, consider any $\lambda_1,\lambda_2\in[0,\overline{\lambda}]$ and let $\pi_{\lambda_1},\pi_{\lambda_2}$ be respective minimizers in $f(\lambda_1)$ and $f(\lambda_2)$. Then, 
        %\begin{align*}
         $   f(\lambda_1)\!\leq\!\mathbb{E}_{\Tilde{x}_0}^{\pi_{{\lambda}_2}}\![ \ell_N(\Tilde{x}_N)\!+\hspace{-0.4em}\sum_{k=0}^{N-1} \hspace{-0.2em}\ell_k(\Tilde{x}_k,u_k)\!+\!\lambda_1(\alpha\!-\!\delta(b_N))]$.
        %\end{align*}
        Further,
            \vspace{-1.5em}
        \begin{align*} %\end{align*}\begin{align*}
            \vspace{-4em}
            f(\lambda_2) &+ |\lambda_1 - \lambda_2| \\&\geq f(\lambda_2) \\&=\mathbb{E}_{\Tilde{x}_0}^{\pi_{{\lambda}_2}}\!\Big[ \ell_N(\Tilde{x}_N)\!+\hspace{-0.4em}\sum_{k=0}^{N-1} \hspace{-0.2em}\ell_k(\Tilde{x}_k,u_k)\!+\!\lambda_1(\alpha-\delta(b_N)) \\&\quad+ (\lambda_2 - \lambda_1)(\alpha-\delta(b_N))\Big] \\
            &= \mathbb{E}_{\Tilde{x}_0}^{\pi_{{\lambda}_2}}\!\Big[ \ell_N(\Tilde{x}_N)\!+\hspace{-0.4em}\sum_{k=0}^{N-1} \hspace{-0.2em}\ell_k(\Tilde{x}_k,u_k)\!+\!\lambda_1(\alpha-\delta(b_N))\Big] \\&\quad+ (\lambda_2 - \lambda_1)\mathbb{E}_{\Tilde{x}_0}^{\pi_{{\lambda}_2}}\!\left[\alpha-\delta(b_N)\right] \\
            &\geq f(\lambda_1) - |\lambda_1 - \lambda_2|,
        \end{align*}
        where the first equality follows by $|\lambda_1 - \lambda_2|$ being non-negative, and the last inequality follows by the initially introduced inequalities and $-1\leq \alpha-\delta(b_N)\leq 1$. Reordering yields 
            $f(\lambda_1) - f(\lambda_2) \leq 2|\lambda_1 - \lambda_2|.$
        By symmetry, 
        $
            |f(\lambda_1) - f(\lambda_2)| \leq 2|\lambda_1 - \lambda_2|,
        $
        showing $f(\lambda)$ is Lipschitz-continuous in $\lambda$. Combined with the fact that $\lambda$ takes values in the compact set $[0,\overline{\lambda}]$, an optimal $\lambda$ is guaranteed to exist \cite{ioffe2005generic}. 
    \end{proof}
\else 
\begin{proof}
        Given any fixed $\lambda\in\mathbb{R}_{\geq 0}$, the existence of an optimal policy for the inner minimization is guaranteed under Assumption \ref{assumption_of_attainability} \cite{schmid2023Jccoc}. Moreover, at least one such optimal policy is deterministic Markov \cite{schmid2023Jccoc}. This allows us to write $\min$ instead of $\inf$ in \eqref{eq_dual_with_binary} and restrict minimization to the class $\Pi$. 
        
        Given the existence of a feasible finite cost policy (Assumption \ref{assumption_of_attainability}), bounds $[0,\overline{\lambda}]\ni\lambda$ can be found \cite{schmid2023Jccoc}. Further, the function 
        \begin{align*}
            f(\lambda)\!=\!\min_{\pi \in \Pi}\mathbb{E}_{\Tilde{x}_0}^\pi\!\left[ \ell_N(\Tilde{x}_N)\!+\hspace{-0.4em}\sum_{k=0}^{N-1} \hspace{-0.2em}\ell_k(\Tilde{x}_k,u_k)\!+\!\lambda(\alpha\!-\!\delta(b_N))\right]
        \end{align*}
        is Lipschitz-continuous in $\lambda$ (CITE ARXIV). 
        Combined, an optimal $\lambda$ is guaranteed to exist \cite{ioffe2005generic}. 
    \end{proof}
\fi 
%Assuming the existence 
%The case $\lambda\rightarrow\infty$ is interpreted as solving for the maximum safe policy. We recover this case using a change of variables $\lambda/(1-\lambda)=\lambda'$ leading to
% \begin{equation}
%     \begin{split}
%         \max_{\lambda\in[0,1]}\min_{\pi \in \Pi_{\text{mix}}} \quad  &\mathbb{E}_{x_0}^\pi\Big[ (1-\lambda)\ell_N(x_N) + \sum_{k=0}^{N-1} (1-\lambda)\ell_k(x_k,u_k)\\ &+\lambda (\alpha-\delta(b_N))\Big] ,
%     \end{split}\label{eq_dual_with_change_of_vars}
% \end{equation}
%where a maximizing argument $\lambda$ is guaranteed to exist, since $\lambda$ lives on a compact set and is linear in the objective function, and a minimizing mixed policy is guaranteed to exist for any $\lambda$ under Assumption \ref{assumption_of_attainability} \cite{schmid2023Jccoc}.

Theorem \ref{cor_max_min_attainable} allows us to replace the supremum and infimum in Problem \eqref{eq_dual_with_binary} with a maximum and minimum. For a fixed $\lambda$, the inner minimization  forms an MDP that is optimally solved by a (not necessarily unique) deterministic Markov policy, obtained via the DP recursion \cite{schmid2023Jccoc}
\begin{align}
\begin{split}
    J_N^{\lambda}(\Tilde{x}_N)&= \ell_N(\Tilde{x}_N) + \lambda(\alpha- \delta(b_N)), \\
    J_k^{\lambda}(\Tilde{x}_k)&=\!\min_{u_k\in\mathcal{U}}\!\ell_k(\Tilde{x}_k,u_k)\!+\hspace{-0.4em}\int_{\Tilde{\mathcal{X}}}\hspace{-0.6em}J_{k+1}^{\lambda}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k).
\end{split}\label{eq_our_dp_recursion_innerdual}
\end{align}
Then, any respective greedy policy on the value functions $J_{0:N}^{\lambda}$ is an optimal argument to the minimization in \eqref{eq_dual_with_binary} \cite{schmid2023Jccoc}. %{\color{red}(recall $\Pi\subseteq\Pi_{\text{mix}}$) \cite{schmid2023Jccoc}. }


%As shown in \cite{schmid2023Jccoc}, Mixing the policies that are obtained over the bisection iterations, a mixed policy with arbitrarily small suboptimality is attained. Note that the results in \cite{schmid2023Jccoc} are derived for the invariance case only, however, our results carry over to reachability and reach-avoid problems under the presented augmented dynamics.  
\begin{definition}
    %Let $\Gamma$ be some policy class. 
    Given $\lambda\in \mathbb{R}_{\geq 0}$, we denote as $\lambda$-optimal under $\Pi$ any policy $\pi_{\lambda}\in\Pi_{\lambda}$ with 
    \begin{align*}
        \Pi_{\lambda}= \Big\{\pi'\in & \ \Pi: \pi'\in{\argmin}_{\pi\in\Pi}  \mathbb{E}_{\Tilde{x}_0}^\pi\big[\ell_N(\Tilde{x}_N) \\ &+ \sum_{k=0}^{N-1} \ell_k(\Tilde{x}_k,u_k)+\lambda (\alpha-\delta(b_N))\big]\Big\}.
    \end{align*}
    %We further denote by $\lambda^{\star}$ any optimal solution to Problem \eqref{eq_dual_of_CCOC} and the associated value functions resulting from \cref{eq_our_dp_recursion_innerdual} under $\lambda^{\star}$ and the policy $\pi_{\lambda^{\star}}$ as $J_{0:N}^{\pi_{\lambda^{\star}}}$
\end{definition}

%Any greedy policy associated to the value functions $J_{0:N}^{{\lambda}}$ resulting from the DP recursion \eqref{eq_our_dp_recursion_innerdual} under $\lambda$ is consequently $\lambda$-optimal. 

%{\color{red} I feel this is the core of the approach, so we should explain it a bit more in detail (space allowing). }
Let $\lambda^{\star}$ be an optimal argument for Problem \eqref{eq_dual_of_CCOC}, then $\Pi_{\lambda^{\star}}$ denotes the set of all $\lambda^{\star}$-optimal deterministic Markov policies for the inner minimization, which also yield optimal arguments in the class of mixed policies. Within $\Pi_{\lambda^{\star}}$, let $\pi_c$ be the policy with the lowest control cost and $\pi_v$ the policy with the highest probability on safety. Then, if Problem \eqref{eq_problemFormulation_CCOC} is feasible, based on \cite{schmid2023Jccoc} the following hold: First, $\pi_v$ is guaranteed to have a safety of at least $\alpha$ and second, an optimal mixed policy to Problem \eqref{eq_problemFormulation_CCOC} can be constructed from $\pi_c$ and $\pi_v$. In the next section, we will design an LP framework that follows this recipe. We first solve for an optimal dual multiplier $\lambda^{\star}$, then we compute the value functions $J_{0:N}^{\lambda^{\star}}$ which implicitly describe the set $\Pi_{\lambda^{\star}}$ and finally we solve for policies $\pi_c$ and $\pi_v$ to construct a mixed policy that solves Problem \eqref{eq_problemFormulation_CCOC} optimally.


%Let the optimal value of $\lambda$ in Problem \eqref{eq_dual_of_CCOC} be given. The set of deterministic Markov policies that solve the DP recursion \eqref{eq_our_dp_recursion_innerdual} optimally under this $\lambda$ hence becomes $\Pi_{\text{dm},\lambda}$. Within $\Pi_{\text{dm},\lambda}$, let $\pi_1$ be the policy with the lowest control cost and $\pi_2$ the policy with the highest probability on achieving the secondary objective. As shown in \cite{schmid2023Jccoc}, one can construct a mixed policy consisting consisting out of $\pi_1$ and $\pi_2$ and this mixed policy solves Problem \eqref{eq_problemFormulation_CCOC} optimally.


%The optimal inputs used in the DP recursion \eqref{eq_our_dp_recursion_innerdual} might not be unique, hence also the optimal policy might not be unique and the set $\Pi_{\lambda^{\star}}$ is not necessarily a singleton. Given the optimal $\lambda$ in Problem \eqref{eq_dual_of_CCOC}, the

\section{Joint Chance Constrained Linear Programming}
\label{sec_jcc_lp}
Consider the LP
% \begin{equation}
%     \begin{split}
%         \sup_{\substack{\lambda\in\mathbb{R}_{\geq 0}, \\J_{0:N}\in \mathcal{M}_{\Tilde{\mathcal{X}}}}  } \quad  &J_0(\Tilde{x}_0)
%         \\ \text{s.t.} \quad &  J_N(\Tilde{x}_N)\leq\ell_N(\Tilde{x}_N) + \lambda(\alpha- \delta(b_N)), \\
%         &J_k(\Tilde{x}_k)\leq  \ell_k(\Tilde{x}_k,u_k)  \\ &\qquad\qquad+ \int_{\Tilde{\mathcal{X}}} J_{k+1}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k),
%     \end{split}
%     \label{eq_lp_ccoc}
% \end{equation}
\begin{equation}
    \begin{split}
        \sup_{\lambda\in\mathbb{R}_{\geq 0}, J_{0:N}\in \mathcal{M}_{\Tilde{\mathcal{X}}}}   \hspace{-1em} &J_0(\Tilde{x}_0)
        \\ \text{s.t.} \quad &  J_N(\Tilde{x}_N)\leq\ell_N(\Tilde{x}_N) + \lambda(\alpha- \delta(b_N)), \\
        &J_k(\Tilde{x}_k)\leq  \ell_k(\Tilde{x}_k,u_k)  \\ &\ \ + \int_{\Tilde{\mathcal{X}}} J_{k+1}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k),
    \end{split}
    \label{eq_lp_ccoc}
\end{equation}
where $\mathcal{M}_{\Tilde{\mathcal{X}}}$ denotes the set of measurable functions from $\Tilde{\mathcal{X}}$ to $\mathbb{R}$ and the constraints hold for all $x_k,x_N\in\Tilde{\mathcal{X}},u_k\in\mathcal{U},k\in[N-1]$. %We pose the following assumptions in addition to Assumption \ref{assumption_of_attainability}. 
% \begin{assumption}
%     There exists a feasible policy for Problem \eqref{eq_problemFormulation_CCOC} with finite cost. 
%     \label{ass_feas_finite_cost_policy}
% \end{assumption}
\begin{lemma}
    Let $\lambda\in\mathbb{R}_{\geq 0}$ be fixed in LP \eqref{eq_lp_ccoc}. Any feasible $J_{0:N}^{\text{\eqref{eq_lp_ccoc}}}$ to LP \eqref{eq_lp_ccoc} yields $J_k^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_k)\leq J_{k}^{{\lambda}}(\Tilde{x}_k)$ for all $k\in[N], \Tilde{x}_k\in\Tilde{\mathcal{X}}$, where $J_{0:N}^{{\lambda}}$ is defined by recursion \eqref{eq_our_dp_recursion_innerdual}. 
    \label{lem_lp_lower_bounds_dp}
\end{lemma}
\begin{proof}
    Since $J_N^{\text{\eqref{eq_lp_ccoc}}}$ is feasible for LP \eqref{eq_lp_ccoc} and by recursion \eqref{eq_our_dp_recursion_innerdual} we have for every $\Tilde{x}_N\in\Tilde{\mathcal{X}}$
    \begin{align*}
        J_N^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_N) \leq \ell_N(\Tilde{x}_N) + \lambda(\alpha-\delta(b_N)) = J_N^{\lambda}(\Tilde{x}_N).
    \end{align*}
    Further, suppose that there exists $k\in[N-1],\Tilde{x}_k\in\Tilde{\mathcal{X}}$ such that $J_k^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_k)> J_k^{\lambda}(\Tilde{x}_k)$. Then, for some input $u_k\in\mathcal{U}$, 
    \begin{align*}
        J_k^{\lambda}(\Tilde{x}_k)&= \ell_k(\Tilde{x}_k,u_k) + \int_{\Tilde{\mathcal{X}}} J_{k+1}^{\lambda}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k)\\ &< J_k^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_k)\\&\leq \ell_k(\Tilde{x}_k,u_k) + \int_{\Tilde{\mathcal{X}}} J^{\text{\eqref{eq_lp_ccoc}}}_{k+1}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k).
    \end{align*}  Since $\Tilde{T}(\cdot|\cdot,\cdot)$ is non-negative, there must exist $\Tilde{x}_{k+1}\in\Tilde{\mathcal{X}}$ where $J_{k+1}^{\lambda}(\Tilde{x}_{k+1})< J_{k+1}^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_{k+1})$. Proceeding inductively up to time step $N$ we obtain that there must exist $\Tilde{x}_N\in\Tilde{\mathcal{X}}$ such that
    $J_N^{\lambda}(\Tilde{x}_N) = \ell_N(\Tilde{x}_N) + \lambda(\alpha-\delta(b_N)) < J_N^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_N)\leq \ell_N(\Tilde{x}_N) + \lambda(\alpha-\delta(b_N)),$
    % \begin{align*}
    %    &J_N^{\lambda}(\Tilde{x}_N) = \ell_N(\Tilde{x}_N) + \lambda(\alpha-\delta(b_N)) \\ &< J_N^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_N)\leq \ell_N(\Tilde{x}_N) + \lambda(\alpha-\delta(b_N)),
    % \end{align*}
    which is a contradiction. Hence, $J_k^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_k)\leq J_k^{\lambda}(\Tilde{x}_k)$ for all $k\in[N],\Tilde{x}_k\in\Tilde{\mathcal{X}}$.
\end{proof}
% \begin{lemma}
%     Under Assumption \eqref{ass_feas_finite_cost_policy}, the supremum in Problem \eqref{eq_lp_ccoc} is attained by some $\lambda\in[0,1],J_{0:N}^{\text{\eqref{eq_lp_ccoc}}}\in \mathcal{M}_{\mathcal{X}}$. \label{lem_lps_attain_maximum}
% \end{lemma}
% \begin{proof}
%     For any $\lambda\in[0,1]$, the value functions $J_{0:N}^{\lambda}$ compute via recursion \eqref{eq_our_dp_recursion_innerdual} yield a feasible solution to Problem \eqref{eq_lp_ccoc}. Further, the yield an upper bound to any feasibl
%     Note that the subgradient of the dual objective \eqref{eq_dual_of_CCOC}  w.r.t. $\lambda$ contains $\alpha - \mathbb{P}_{x_0}^{\pi_{\lambda}}(x_{0:N}\in \mathcal{H}))$. Under Assumption \eqref{ass_feas_finite_cost_policy}, Problem \eqref{eq_problemFormulation_CCOC} is feasible, hence the maximum safety is at least $\alpha$. If it is exactly $\alpha$, then the subgradient becomes zero under the maximum safe policy, which is obtained from the DP recursion \eqref{eq_our_dp_recursion_innerdual} under $\lambda=1$. Combined with the objective function being concave, $\lambda=1$ must be an optimal argument. If there exists a finite cost policy with a success probability greater than $\alpha$, an optimal $\lambda\in[0,1)$ is guaranteed to exist by \cite[Proposition~5.2]{schmid2023Jccoc}. In either case the resulting policy $\pi_{\lambda}$ yields the inner minimum in Problem \eqref{eq_dual_of_CCOC} and measurable associated value functions  $J_{0:N}^{\pi_{\lambda}}(\cdot)$ \cite{schmid2023Jccoc}.
% \end{proof}
\begin{theorem}
    The supremum in LP \eqref{eq_lp_ccoc} is attained by some $\lambda\in\mathbb{R}_{\geq 0},J_{0:N}^{\text{\eqref{eq_lp_ccoc}}}\in \mathcal{M}_{\Tilde{\mathcal{X}}}$. An optimal argument $\lambda$ of the LP \eqref{eq_lp_ccoc} is also optimal for Problem \eqref{eq_dual_of_CCOC} and vice versa.
    \label{thm_optimal_lambda}
\end{theorem}
\begin{proof}
    Fix any $\lambda\in\mathbb{R}_{\geq 0}$. Then, by Lemma \ref{lem_lp_lower_bounds_dp} any feasible solution of the LP yields a lower bound to the DP solution $J_{0:N}^{{\lambda}}(\cdot)$. Further, $J_{0:N}^{{\lambda}}(\cdot)$ are measurable functions by \cite{schmid2023Jccoc} and satisfy the constraints in LP \eqref{eq_lp_ccoc}. Hence, under the fixed $\lambda$, they are an optimal solution of the LP. 

    Let $\Lambda^{\star}$ denote the set of optimal values for $\lambda$ in Problem \eqref{eq_dual_of_CCOC}, i.e., the maximum value of $J_{0}^{\lambda}(\Tilde{x}_0)$ is achieved if and only if $\lambda\in\Lambda^{\star}$. 
    Fix any $\lambda'\notin\Lambda^{\star}$ in LP \eqref{eq_lp_ccoc} and let $\lambda^{\star}\in\Lambda^{\star}$. Then, $J_{0}^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_0)\leq J_{0}^{\lambda'}(\Tilde{x}_0)$ by Lemma \ref{lem_lp_lower_bounds_dp} and $J_{0}^{\lambda'}(\Tilde{x}_0)< J_{0}^{\lambda^{\star}}(\Tilde{x}_0)$. Combined, $J_{0}^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_0)< J_{0}^{\lambda^{\star}}(\Tilde{x}_0)$ and together with $(\lambda^{\star},J_{0:N}^{\lambda^{\star}})$ being feasible in LP \eqref{eq_dual_of_CCOC} $J_{0:N}^{\text{\eqref{eq_lp_ccoc}}}$ is a suboptimal solution to LP \eqref{eq_dual_of_CCOC}. Hence, any optimal $\lambda$ in \eqref{eq_lp_ccoc} must be contained in $\Lambda^{\star}$. Vice versa, any $\lambda^{\star}\in\Lambda^{\star}$ is optimal to LP \eqref{eq_lp_ccoc} since $(\lambda^{\star},J_{0:N}^{\lambda^{\star}})$ is a feasible and optimal solution that attains the greatest possible value of $J_{0}^{\lambda^{\star}}(\Tilde{x}_0)$.
    % By Lemma \ref{lem_lp_lower_bounds_dp}, $J_{0}^{\lambda^{\star}}(\Tilde{x}_0)$ is an upper bound to the LP solution $J_{0}^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_0)$, which, at the same time, is feasible. Hence,  $(\lambda^{\star},J_{0:N}^{\lambda^{\star}})$ is an attainable optimal solution. Summarizing, any optimal argument $\lambda$ must be contained in $\Lambda^{\star}$ and the supremum in LP \eqref{eq_lp_ccoc} is attained. Any optimal $\lambda^{\star}\in\Lambda^{\star}$ being optimal for LP \eqref{eq_lp_ccoc} follows by $(\lambda^{\star},J_{0:N}^{\lambda^{\star}})$ being feasible.
    %Assume $\lambda'\notin\Lambda^{\star}$, $\lambda^{\star}\in\Lambda^{\star}$, then $J_{0}^{\text{\eqref{eq_lp_ccoc}}}(x_0)\leq J_{0}^{\lambda'}(x_0)< J_{0}^{\lambda^{\star}}(x_0)$ yields a suboptimal solution. Hence, $J_{0}^{\text{\eqref{eq_lp_ccoc}}}(x_0)$ attains its maximum if and only if  $\lambda\in\Lambda^{\star}$ and equals $J_{0}^{\star}(x_0)$. 
\end{proof}


% The reason is that the value functions in Problem \eqref{eq_lp_ccoc} may not be maximized whenever they do not bound the optimal value $J_0^{\text{\eqref{eq_lp_ccoc}}}(x_0)$. For instance consider states $\Tilde{x}_{k+1}$ where $J_{k+1}^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_{k+1})<J_{k+1}^{\lambda}(\Tilde{x}_{k+1})$ and which, from some $\Tilde{x}_k$, have zero $T$-measure under some optimal input $u_1$ and non-zero $T$-measure under some suboptimal input $u_2$. Then, it might be that
% \begin{align*}
%     J_{k}^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_k) &=    \ell_k(\Tilde{x}_k,u_1) + \int_{\Tilde{\mathcal{X}}} J_{k+1}^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_{k+1})T(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_1)
%     \\&=\ell_k(\Tilde{x}_k,u_1) + \int_{\Tilde{\mathcal{X}}} J_{k+1}^{\lambda}(\Tilde{x}_{k+1})T(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_1), \\
%     J_{k}^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_k) & =   \ell_k(\Tilde{x}_k,u_2) + \int_{\Tilde{\mathcal{X}}} J_{k+1}^{\text{\eqref{eq_lp_ccoc}}}(\Tilde{x}_{k+1})T(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_2) \\&< \ell_k(\Tilde{x}_k,u_2) + \int_{\Tilde{\mathcal{X}}} J_{k+1}^{\lambda}(\Tilde{x}_{k+1})T(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_2).
% \end{align*}



%The value $J_0(x_0)$ might be bounded by some optimal input $u_1$ and the value function at any state with non-zero $T$-measure under $u_1$ must clearly be maximized to not yield the least restrictive bound. For any zero $T$-measure state under $u_1$, however, the value function might be arbitrary, as long as any suboptimal input, say $u_2$ appears more tight than $u_1$. Hence, two inputs $u_1$, $u_2$ might appear equally optimal since the value function may not be maximized at every state, although $u_2$ might be strictly suboptimal. 


While the above Theorem guarantees that the optimal arguments for $\lambda$ in LP \eqref{eq_lp_ccoc} and Problem \eqref{eq_dual_of_CCOC} are equivalent, this is not necessarily true for the value functions $J_{0:N}^{\text{\eqref{eq_lp_ccoc}}}$ and $J_{0:N}^{\lambda}$. Hence, greedy policies for $J_{0:N}^{\text{\eqref{eq_lp_ccoc}}}$ advertise potentially suboptimal inputs, making $J_{0:N}^{\text{\eqref{eq_lp_ccoc}}}$ useless for constructing an optimal solution for Problem \eqref{eq_problemFormulation_CCOC} \cite{schmid2022probabilistic}. We address this issue by solving a second LP, keeping $\lambda$ fixed to its optimal value $\lambda^{\star}$ from LP \eqref{eq_lp_ccoc} and including the value functions $J_{0:N}$ in the objective via a non-negative measure $\nu$ that assigns positive
mass to all open subsets of $\Tilde{\mathcal{X}}$:
\begin{equation}
    \begin{split}
        \max_{J_{0:N}\in \mathcal{M}_{\Tilde{\mathcal{X}}}} \quad  &J_0(\Tilde{x}_0)+\sum_{k=1}^N\int_{\Tilde{\mathcal{X}}}J_k(\Tilde{x}_k)\nu(dx_k)
        \\ \text{s.t.} \quad &J_N(\Tilde{x}_N)\leq\ell_N(\Tilde{x}_N) + \lambda^{\star}(\alpha- \delta(b_N)), \\
        &J_k(\Tilde{x}_k)\leq  \ell_k(\Tilde{x}_k,u_k) + \\ & \ \quad \qquad \int_{\Tilde{\mathcal{X}}} J_{k+1}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k),
    \end{split}\label{eq_lp_ccoc_value_functions}
\end{equation}
where the constraints hold for all $\Tilde{x}_k,\Tilde{x}_N\in\Tilde{\mathcal{X}},u_k\in\mathcal{U},k\in[N-1]$. We denote the optimal arguments as $J_{0:N}^{\text{\eqref{eq_lp_ccoc_value_functions}}}$. The existence of the maximum follows as in Theorem \ref{thm_optimal_lambda}. %Following the discussion in \cite{schmid2022probabilistic}, the optimal arguments of the linear program are ($\nu$-a.e.) equivalent to the value functions obtained with the DP recursion.
\begin{theorem}
\label{thm_lp_solution_optimal}
    Let $\lambda^{\star}$ denote the optimal argument of $\lambda$ in LP \eqref{eq_lp_ccoc}. The value functions $J_{0:N}^{\text{\eqref{eq_lp_ccoc_value_functions}}}$ obtained as the optimal argument of LP \eqref{eq_lp_ccoc_value_functions} are upper bounded by $J_{0:N}^{\lambda^{\star}}$ obtained by the DP recursion \eqref{eq_dual_of_CCOC} and are $\nu$-almost-everywhere equivalent. The values $J_{0}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_0) = J_{0}^{\star}(\Tilde{x}_0)$ are equivalent.
\end{theorem}
\begin{proof}
    The fact $J_{0:N}^{\text{\eqref{eq_lp_ccoc_value_functions}}}\leq J_{0:N}^{\lambda^{\star}}$ can be established as in Lemma \ref{lem_lp_lower_bounds_dp} by $J_{0:N}^{\lambda^{\star}}$ being feasible for LP \eqref{eq_lp_ccoc_value_functions}. If there is a non-zero $\nu$-measure set of states where the LP solution is strictly suboptimal or if $J_0^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_0)$ is strictly suboptimal, then 
    $        J_0^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_0)\!+\!\sum_{k=1}^N\!\int_{\Tilde{\mathcal{X}}}\!J_k^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_k)\nu(d\Tilde{x}_k)\!<\!J_0^{\lambda^{\star}}(\Tilde{x}_0)\!+\!\sum_{k=1}^N\!\int_{\Tilde{\mathcal{X}}}\!J_k^{\lambda^{\star}}(\Tilde{x}_k)\nu(d\Tilde{x}_k)
        $
    % \begin{align*}
    %     &J_0^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_0)+\sum_{k=1}^N\int_{\Tilde{\mathcal{X}}}J_k^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_k)\nu(d\Tilde{x}_k) \\ < & \ J_0^{\lambda^{\star}}(\Tilde{x}_0)+\sum_{k=1}^N\int_{\Tilde{\mathcal{X}}}J_k^{\lambda^{\star}}(\Tilde{x}_k)\nu(d\Tilde{x}_k)
    % \end{align*}
    and, by feasibility of $J_{0:N}^{\lambda^{\star}}$, $J_{0:N}^{\text{\eqref{eq_lp_ccoc_value_functions}}}$ is not an optimal solution of the LP. Hence, $J_{0:N}^{\text{\eqref{eq_lp_ccoc_value_functions}}}$ can not be smaller than  $J_{0:N}^{\lambda^{\star}}$ for a non-zero $\nu$-measure set of states and not larger by the prior bound, leading to the claim.
\end{proof}

% Informal: However, the resulting value functions give us no information about the optimal policy. The reason is that there might be a set of states that are never reached under the truely optimal inputs. Hence, the value of the value function at these states may be lower than what the they should be and, worst case, suptoptimal inputs appear optimal under the greedy policy. The good thing is, that we have $\lambda^*$, which defines a standard MDP that we need to solve.
% Therefore, we run a second linear program
% \begin{equation}\label{eq_lp_ccoc}
%     \begin{split}
%         \sup_{J_{0:N}\in ? } \quad  &J_0(x_0)+\sum_{k=1}^N\int_{\Tilde{\mathcal{X}}}J_k(x_k)dx_k
%         \\ s.t. &J_N(\Tilde{x}_N)=\ell_N(\Tilde{x}_N) - \lambda^{\star} \delta(b_N), \\
%         J_k(\Tilde{x}_k)&\leq  \ell_k(\Tilde{x}_k,u_k) + \\ &\quad \int_{\Tilde{\mathcal{X}}} J_{k+1}(\Tilde{x}_{k+1})T(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k),
%     \end{split}
% \end{equation}
% where $\lambda^*$ is the optimal solution of the prior LP. Now, there might be a zero Lebesgue measure set of states with suboptimal values. 

\begin{assumption}
    For every $\Tilde{x}\in\Tilde{\mathcal{X}},u´\in\mathcal{U}$, the kernel $\Tilde{T}(\cdot|\Tilde{x},u)$ is absolutely continuous with respect to $\nu$. 
    \label{ass_T_abs_cont}
\end{assumption}
\begin{proposition}
    Under Assumption \ref{ass_T_abs_cont}, the set of greedy policies with respect to $J_{0:N}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_0)$ is equivalent to the set of greedy policies with respect to $J_{0:N}^{\lambda^{\star}}(\Tilde{x}_0)$.
\end{proposition}
\begin{proof}
    For $k\in[N]$, let $\mathcal{C}_k=\{\Tilde{x}\in\Tilde{\mathcal{X}}|J_{k}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_k)< J_{k}^{\lambda^{\star}}(\Tilde{x}_k)\}$, which has zero $\nu$-measure by \cref{thm_lp_solution_optimal}. Then, for $k\in[N-1]$ the greedy policy picks 
    %\vspace{-.15cm}
    \begin{align*}
        &\argmin_{u_k\in\mathcal{U}}\int_{\Tilde{X}}J_{k+1}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k)
        \\=&\argmin_{u_k\in\mathcal{U}}\int_{\Tilde{X}\setminus\mathcal{C}_{k+1}}\hspace{-2em}J_{k+1}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) 
    \\=&\argmin_{u_k\in\mathcal{U}}\int_{\Tilde{X}\setminus\mathcal{C}_{k+1}}\hspace{-2em}J_{k+1}^{\lambda^{\star}}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k)
        \\=&\argmin_{u_k\in\mathcal{U}}\int_{\Tilde{X}}J_{k+1}^{\lambda^{\star}}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k),
    \end{align*} since $\mathcal{C}_{k+1}$ is associated zero $\nu$-, hence, zero $\Tilde{T}$-measure.
    %
    % For the second statement, assume there is a suboptimal input $u_k'$ that forms an active constraint, then
    % \begin{align*}
    %     J_k^{\text{\eqref{eq_lp_ccoc_value_functions}}}(x_k)&\leq\min_{u_k\in\mathcal{U}}\ell_k(\Tilde{x}_k,u_k) + \int_{\Tilde{\mathcal{X}}} J_{k+1}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_{k+1})T(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k)  
    %     \\&<  \ell_k(\Tilde{x}_k,u_k') + \int_{\Tilde{\mathcal{X}}} J_{k+1}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_{k+1})T(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k') = J_k^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_k).
    % \end{align*}
    % Assume there is an optimal input $u_k'$ that does not form an active constraint, then 
    % \begin{align*}
    %     J_k^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_k) &< \ell_k(\Tilde{x}_k,u_k') + \int_{\Tilde{\mathcal{X}}} J_{k+1}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_{k+1})T(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k')  
    %     \\&=\min_{u_k\in\mathcal{U}}  \ell_k(\Tilde{x}_k,u_k) + \int_{\Tilde{\mathcal{X}}} J_{k+1}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_{k+1})T(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k').
    % \end{align*}
    % Clearly, both statements form a contradiction.
\end{proof}

In summary, solving the LP \eqref{eq_lp_ccoc} returns the optimal dual multiplier $\lambda^{\star}$. Subsequently solving the LP \eqref{eq_lp_ccoc_value_functions} under $\lambda^{\star}$ returns the value functions $J_{0:N}^{\text{\eqref{eq_lp_ccoc_value_functions}}}$, whose greedy policies correspond to the set of $\lambda^{\star}$-optimal policies. Following \cite{schmid2023Jccoc}, the optimal mixed policy for Problem \eqref{eq_problemFormulation_CCOC} can now be constructed by interpolating the cheapest and safest $\lambda^{\star}$-optimal deterministic Markov policies, denoted $\pi_{c,\lambda^{\star}}$, $\pi_{v,\lambda^{\star}}$, respectively. These can be computed using the recursions \eqref{eq_max_cost_evaluation} and \eqref{eq_max_invariance_evaluation}, restricting to inputs that are also optimal under $J_{0:N}^{\text{\eqref{eq_lp_ccoc_value_functions}}}$, e.g., the safest $\lambda^{\star}$-optimal policy can be computed with the recursion 
\begin{align}
\begin{split}
        V_{v,N}^{\star}(\Tilde{x}_N) \!&=\hspace{-0.1em}\mathbb{1}_{\mathcal{A}}(\Tilde{x}_N),  \\
        V_{v,k}^{\star}(\Tilde{x}_k)\!&=\hspace{-0.4em}\sup_{u_k\in\mathcal{U}} \mathbb{1}_\mathcal{A}(\Tilde{x}_k)\int_{\Tilde{\mathcal{X}}}\hspace{-0.4em}V_{v,k+1}^{\star}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_{k}, u_k),\\
        &\ \hspace{0.8em}\text{s.t.} \int_{\Tilde{X}}\hspace{-0.4em}J_{k+1}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) \\&\ \hspace{1.8em}= \argmin_{u'\in\mathcal{U}}\int_{\Tilde{X}}\hspace{-0.4em}J_{k+1}^{\text{\eqref{eq_lp_ccoc_value_functions}}}(\Tilde{x}_{k+1})\Tilde{T}(d\Tilde{x}_{k+1}|\Tilde{x}_k,u'),
\end{split}
\label{eq_safety_evaluation_of_lambda_optimal}
\end{align}
for $k\in[N-1]$. The constraint is continuous in $u_k$ since $\Tilde{T}$ is continuous in $u_k$ given a fixed $\Tilde{x}_k$. Hence, the level set described by the constraint is closed. Intersected with the constraints described by the compact set $\mathcal{U}$, the constraints are compact. Since the objective function is continuous in $u_k$ given $\Tilde{x}_k$, the supremum is always attained by some input $u_k$ \cite{ioffe2005generic}. A similar recursion can be formulated based on \eqref{eq_max_cost_evaluation} to compute the cheapest $\lambda^{\star}$-optimal policy $\pi_{c,\lambda^{\star}}$. 

Let the associated safety of the policies $\pi_{c,\lambda^{\star}}$ and $\pi_{v,\lambda^{\star}}$ at $x_0$ be denoted by $v_{c}$ and $v_{v}$, respectively. Under Assumption \ref{assumption_of_attainability} and based on \cite{schmid2023Jccoc}, the policy $\pi_{v,\lambda^{\star}}$ will have a safety of at least $\alpha$ and constructing a mixed policy that samples 
\begin{align}
\pi_{\text{mix}}=\begin{cases}
\pi_{v,\lambda^{\star}} & \text{with probability } p_{v}\!=\!\frac{\alpha - v_{c}}{v_{v} - v_{c}}, \\
\pi_{c,\lambda^{\star}} & \, \text{otherwise,}
\end{cases}
\label{eq_stochastic_policies_ratios}
\end{align}
yields an optimal mixed policy to Problem \eqref{eq_problemFormulation_CCOC}. To summarize, the algorithmic steps are given in \cref{alg_final}.


\begin{algorithm}[!tbp]
\caption{Joint Chance Constr. Optimal Control}
%\KwData{$\mathcal{X},\mathcal{U},T,N,\tilde{x}_0,\alpha, \Delta$}
%\texttt{\\}
$\lambda^{\star}\leftarrow$ LP \eqref{eq_lp_ccoc}\;
$J_{0:N}^{\eqref{eq_lp_ccoc_value_functions}} \leftarrow$ LP \eqref{eq_lp_ccoc_value_functions}\;
$(\pi_{c,\lambda^{\star}}) \leftarrow$ Recursion \eqref{eq_max_cost_evaluation} s.t. greedy on $J_{0:N}^{\text{\eqref{eq_lp_ccoc_value_functions}}}$\;
$v_{c} \leftarrow$ Recursion \eqref{eq_invariance_evaluation} s.t. $\pi_{c,\lambda^{\star}}$\;
$(\pi_{v,\lambda^{\star}},v_{v}) \leftarrow$ Recursion \eqref{eq_max_invariance_evaluation} s.t. greedy on $J_{0:N}^{\text{\eqref{eq_lp_ccoc_value_functions}}}$\;
%$c_{v} \leftarrow$ Recursion \eqref{cost_DP} s.t. $\pi_{v,\lambda^{\star}}$\;
$p_v\leftarrow$ Eq. \eqref{eq_stochastic_policies_ratios}\;
return $\pi_{c,\lambda^{\star}},\pi_{v,\lambda^{\star}},p_v$\;
\label{alg_final}
\end{algorithm}

%Our results trivially extend to the case of finite state and input spaces.



% Defining $\Tilde{x}_{k}=\begin{bmatrix}
%     x_k & b_k
% \end{bmatrix}^{\top}$ the combined transition kernel, by overloading the function $T$, reads as 
% \begin{align*}
%     &T(\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) \\&= \begin{cases}
%     T(x_{k+1}|x_k,u_k) & \text{if} \ b_{k}=0 \land b_{k+1}=0 \lor b_{k+1}=\mathbb{1}_{\mathcal{A}}(x_{k+1}) \\
%     0 & \text{otherwise}.
% \end{cases}
% \end{align*}
% One can equivalently formulate this transition kernel as 
% \begin{align*}
%     T(\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) &= 
%     T(x_{k+1}|x_k,u_k) \big((1-b_{k})(1-b_{k+1}) \\& \quad + (1-|b_{k+1}-\mathbb{1}_{\mathcal{A}} (x_{k+1})|)\big),
% \end{align*}
% which is measurable since the absolute value of a measurable function and a point-wise product of measurable functions are measurable.

 



% The goal of this section is to derive a tractable linear programming framework for solving optimal control problems with reachability, invariance and reach-avoid constraints.

% To ease notation, we introduce the path formulas $\Phi_I(\mathcal{A}), \Phi_R(\mathcal{T}), \Phi_{RA}(\mathcal{A},\mathcal{T})$ that define invariance, reachability and reach-avoid specifications on the trajectory $x_{0:N}$. Whether these logical statements are satisfied for a given trajectory $x_{0:N}$ can then easily be evaluated in terms of products of set indicator functions. 
% \begin{align}
% \begin{split}
%     x_{0:N}\models\Phi_I(\mathcal{A}) &=\prod_{k=0}^N\mathbb{1}_{\mathcal{A}}(x_k) \\
%     x_{0:N}\models\Phi_R(\mathcal{T}) 
%     &=1-\prod_{k=0}^N(1-\mathbb{1}_{\mathcal{T}}(x_k)) \\
%     x_{0:N}\models\Phi_{RA}(\mathcal{A},\mathcal{T}) &=1-\prod_{k=0}^N\left(1-\mathbb{1}_{\mathcal{T}}(x_k)\prod_{i=0}^k\mathbb{1}_{\mathcal{T}}(x_i) \right) 
% \end{split}
% \label{eq_secSpecs_based_on_prod_of_indicator}
% \end{align}

% Furthermore, the probability of satisfying a path formula for a stochastic evolution of the trajectory is given by (\cite{abate2008probabilistic}, \cite{kariotoglou2017linear})
% \begin{align*}
%     P(x_{0:N}\models\Phi_I(\mathcal{A}))&=\mathbb{E}\left[x_{0:N}\models\Phi_I(\mathcal{A})\right] \\
%     P(x_{0:N}\models\Phi_R(\mathcal{T}) )&=\mathbb{E}\left[x_{0:N}\models\Phi_R(\mathcal{A})\right] \\
%     P(x_{0:N}\models\Phi_{RA}(\mathcal{A},\mathcal{T}))&=\mathbb{E}\left[x_{0:N}\models\Phi_{RA}(\mathcal{A},\mathcal{T})\right].
% \end{align*}

% \subsection{Lagrange Dual Formulation}
% Following the precedure in \cite{schmid2023Jccoc} we aim to evaluate the Lagrange dual of problem \eqref{eq_problemFormulation_CCOC}
% \begin{equation}\label{eq_lagrange_dual_over_stochasticCausal_0}
%     \begin{split}
%         \max_{\lambda_{1:M} \in \mathbb{R}_{\geq0}} \inf_{\pi \in \Pi_{sc}}\! &\mathbb{E}_{x_0}^\pi\!\left[ \ell_N(x_N)\!+\!\sum_{k=0}^{N-1}\!\ell_k(x_k,\mu_k(x_k))\right]
%          \\&+ \sum_{i=1}^M\lambda_i(p_i\!-\!\mathbb{P}(x_{0:N}\models \Phi_i)).
%      \end{split}
% \end{equation}
% While it is tempting to solve the inner optimization problem via dynamic programming, the terms $\mathbb{P}(x_{0:N}\models \Phi_i)$ yield a product over all time steps in the cost function. This information might only be available fully at the terminal time $N$, yet formulating the dynamic programming recursion to recall the full past trajectory is computationally intractable. 

% Fortunately, it is not necessary to have knowledge of the full trajectory to verify if invariance, reachability, or reach-avoid specifications have been violated or satisfied. In fact, the only information that is needed is whether a trajectory left an invariant set, reached a target set, or reached a target set before leaving an invariant set - binary information that can be captured in an augmented state with respective dynamics.

% For any invariance specification, let the state be augmented by a binary state $b_k^I$ with $b_0 = \mathbb{1}_{\mathcal{A}}(x_0)$ and dynamics $b_{k+1}^I=\mathbb{1}_{\mathcal{A}}(x_{k+1})b_k^I$, then $\prod_{k=0}^N\mathbb{1}_{\mathcal{A}}(x_k) = b_N^I$. Defining $\Tilde{x}_{k}=\begin{bmatrix}
%     x_k & b_k
% \end{bmatrix}^{\top}$ the combined transition kernel, by overloading the function $T$, reads as 
% \begin{align*}
%     &T(\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) \\&= \begin{cases}
%     T(x_{k+1}|x_k,u_k) & \text{if} \ b_{k}=0 \land b_{k+1}=0 \lor b_{k+1}=\mathbb{1}_{\mathcal{A}}(x_{k+1}) \\
%     0 & \text{otherwise}.
% \end{cases}
% \end{align*}
% One can equivalently formulate this transition kernel as 
% \begin{align*}
%     T(\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) &= 
%     T(x_{k+1}|x_k,u_k) \big((1-b_{k})(1-b_{k+1}) \\& \quad + (1-|b_{k+1}-\mathbb{1}_{\mathcal{A}} (x_{k+1})|)\big),
% \end{align*}
% which is measurable since the absolute value of a measurable function and a point-wise product of measurable functions are measurable.

%  Similarly for reachability problems, define $b_0^R = \mathbb{1}_{\mathcal{T}}(x_0)$ with $b_{k+1}^R=\mathbb{1}_{\mathcal{T}}(x_k) + (1-\mathbb{1}_{\mathcal{T}}(x_k))b_k^R$ and
%  \begin{align*}
%     &T(\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) \\&= \begin{cases}
%     T(x_{k+1}|x_k,u_k) & \text{if} \ b_{k}=1 \land b_{k+1}=1 \lor b_{k+1}=\mathbb{1}_{\mathcal{T}}(x_{k+1}) \\
%     0 & \text{otherwise}.
% \end{cases}
% \end{align*} For reach-avoid problems define the ternary variable $b_k^{RA}\in\{0,1,2\}$ with $b_0^{RA} = \mathbb{1}_{\mathcal{T}}(x_0)$ and 
% \begin{align*}
%     b_{k+1}^{RA} = \begin{cases}
%     0, & b_k=0 \lor x_{k+1}\notin\mathcal{A} \\
%     1, & b_k=1 \land  x_{k+1}\in\mathcal{A} \land x_{k+1}\notin\mathcal{T} \\
%     2, & b_k=2 \lor  x_{k+1}\notin\mathcal{T} 
%     \end{cases}
% \end{align*}
% such that
%  \begin{align*}
%     &T(\Tilde{x}_{k+1}|\Tilde{x}_k,u_k) \\&= \begin{cases}
%     T(x_{k+1}|x_k,u_k) & \text{if} \ b_{k}=2 \land b_{k+1}=2 \lor \\ &b_k=1 \land b_{k+1}=\mathbb{1}_{\mathcal{T}}(x_{k+1})+\mathbb{1}_{\mathcal{A}\cup\mathcal{T}}(x_{k+1})\\
%     0 & \text{otherwise}.
% \end{cases}
% \end{align*}
% Furthermore, we define the success indicator function $\delta$. For invariance and reachability specifications
% \begin{align*}
%     \delta(b_k)=\begin{cases}
%     1 & \text{if }b_k=1\\ 
%     0 &  \text{else, }
% \end{cases}
% \intertext{and for reach-avoid specifications}
% \delta(b_k)=\begin{cases}
%     1 & \text{if }b_k=2\\ 
%     0 &  \text{else. }
% \end{cases}
% \end{align*}
% Under this definition, we have $\mathbb{P}(x_{0:N}\models \Phi_i) = \mathbb{E}_{x_0}^\pi\left[\delta_i(b_{i,N})\right]$ (maybe we need a formal proof here? Or formalize the derivation of before?)


% If multiple secondary objectives are defined, accordingly many variables may be added and the transition kernel adjusted. The only limitation is that the state space increases exponentially with the number of specifications, and likewise the computational complexity of our solution.  

% For $M$ secondary specifications, let 
% $\Tilde{x}_k=\begin{bmatrix}
%     x_k & b_{1,k} & \dots & b_{M,k}
% \end{bmatrix}^{\top}$ be the resulting state. This allows us to write Problem \eqref{eq_lagrange_dual_over_stochasticCausal_0} as
% \begin{equation}\label{eq_lagrange_dual_with_secondary_vars}
%     \begin{split}
%         \max_{\lambda_{1:M} \in \mathbb{R}_{\geq0}} \inf_{\pi \in \Pi_{sc}}\! &\mathbb{E}_{x_0}^\pi\!\Big[ \ell_N(x_N)\!+\!\sum_{k=0}^{N-1}\!\ell_k(x_k,\mu_k(x_k))
%          \\&+ \sum_{i=1}^M\lambda_i(p_i\!-\!\delta_i(b_{i,N}))\Big].
%      \end{split}
% \end{equation}
% We now aim to formulate problem \eqref{eq_lagrange_dual_with_secondary_vars} as a linear programming problem. 

% Following the procedure of \cite{schmid2023Jccoc}, let us fix $\lambda_{1:M}$ and note that the inner problem can be solved by the dynamic programming recursion 
% \begin{align}
% \begin{split}
%     J_N^*(\Tilde{x}_N)&= \ell_N(\Tilde{x}_N) - \sum_{i=1}^M\lambda_i \delta_i(b_{i,N}), \\
%     J_k^*(\Tilde{x}_k)&= \min_{u_k\in\mathcal{U}} \ell_k(\Tilde{x}_k,u_k) + \\ &\quad \int_{\Tilde{\mathcal{X}}} J_{k+1}^*(\Tilde{x}_{k+1})T(d\Tilde{x}_{k+1}|\Tilde{x}_k,u_k),
% \end{split}\label{eq_our_dp_recursion_innerdual}
% \end{align}
% where the value of the inner minimization in problem \eqref{eq_lagrange_dual_over_stochasticCausal_0} equals $J_0^*(x_0)$ and the optimal arguments define a deterministic, causal, but not necessarily unique policy.

% Instead of solving for $J_0^*(x_0)$ via dynamic programming, we can utilize the linear programming formulation [cite Bertsekas or lerma book]
% \begin{align*}
%     \max_{J_{0:N}} &&J_0(x_0)
%          \\&\text{s.t.} && J_{k}(x_{k})\leq l_k(x_k,u_k) + \int_{\mathcal{X}}J_{k+1}(x_{k+1})T(dx_{k+1}|x_k,u_k)  \\
%          &&& J_N(x_N) = l_N(x_N) - \sum_{i=1}^M\lambda_i \delta_i(b_{i,N})
% \end{align*}
% Combined with the bilevel optimization, we obtain
% \begin{align*}
%     &\max_{\lambda_{1:M} \in \mathbb{R}_{\geq0}} \min_{\pi \in \Pi_{sc}}&&\mathbb{E}_{x_0}^\pi\!\left[ \ell_N(x_N)\!+\!\sum_{k=0}^{N-1}\!\ell_k(x_k,\mu_k(x_k))\right]
%          \\&&&+ \lambda(p_s\!-\!\mathbb{P}_{x_0}^\pi(x_{0:N}\in \mathcal{A})) \\
%     =&\max_{\lambda_{1:M} \in \mathbb{R}_{\geq0}, J_{0:N}} &&J_0(x_0)
%          \\&\text{s.t.} && J_{k}(x_{k})\leq l_k(x_k,u_k) + \int_{\mathcal{X}}J_{k+1}(x_{k+1})T(dx_{k+1}|x_k,u_k)  \\
%          &&& J_N(x_N) = l_N(x_N) - \sum_{i=1}^M\lambda_i \delta_i(b_{i,N}),\label{eq_Lp_formulation}
% \end{align*}
% where the constraints hold for all $x_k,x_N\in\Tilde{\mathcal{X}}, u_k\in\mathcal{U}, k\in[N-1]$. 

% We next proof that any policy optimal for Problem \eqref{eq_problemFormulation_CCOC} is also optimal for \eqref{eq_Lp_formulation}. Furthermore, there exist $M$ deterministic, causal, not necessarily distinct, optimal policies for problem \eqref{eq_Lp_formulation} that can be used to generate a mixed policy that is optimal for Problem \eqref{eq_problemFormulation_CCOC}.


% First note that there exists a stochastic causal policy that is optimal under lambda, meets the constraints and has minimum cost. This follows by the duality arguments (at the optimal lambda, zero lies in the subgradient, and at this point there exists a solution satisfying the constraint, check out last p









% per for this).


% Let there be a stochastic causal policy that is optimal. Then there also exists a mixed policy that is optimal. This mixed policy must consist of optimal deterministic causal policies. 











% Argue with lagrangians (meaning of optimum lambda). Then same proof as other paper. Assume lambda optimal. Assume there is policy cheaper and better in all constraints. Then policy not optimal. Assume there exists policy that is cheaper in cost and safer in at least one constraint while not violating others. Then policy not optimal. Assume 


















% To generate mixed policies with arbitrarily small suboptimality, we generate two perturbations $\lambda_1<\lambda<\lambda_2$ and resolve the inner minimization. Evaluating the safety of the policies associated to the value functions we can pick the right mixing.

% Add discussion that this works because of monotonicity (refer to last paper). Suboptimality due to epsilon...

% \begin{proof}
%     Show this solves our problem to optimality by building connection to results.
% \end{proof}





% Guarantees when using ADP (Peyman and Tobias paper)? -> We have probabilistic guarantees on the optimal value. We can then argue based on lambda how much safety margin we might miss and tighten our constraints accordingly. This would require that we know a-priori how much error we might obtain by going for the adp case -> Might be very hard. Peyman paper is AC infinite horizon. We can still use Kariotoglou guarantees, but this only gives us information that few states are bad, but not how bad.

% Discuss with Tobias:
% First error of ADP: Richness of function class (Beuchat paper)
% Second error of ADP: Sampling -> Suboptimal value function and policy -> Kariotoglou: Guarantee that only few states bad, but how bad unclear, Tobias: AC problem, probabilistic bound on suboptimality of value function -> Use Beuchat paper to infer suboptimality of policy once we know supoptimality of the value function(?)
% -> Ideally we could use the bound of the misestimate to tighten our safety constraints such that we can guarantee the original safety constraint, but we have no means to estimate the first error. -> Not true. If we have Lipschitz bounds on the value function we can get an upper bound on this error for sure (and we can probably guarantee this with the binary separation of the state space).

% If all of this does not work, just use Kariotoglou guarantees


% Discretization: Add error bounds for discrete setting: Compute subgradient as usual by evaluating safety for discretized MDP. -> Safety guaranteed. No suboptimality bound (yet) since we would have to think about error introduced by tightening of constraints (which should be easy by geometric construction) and by Lipschitz constant of stage cost (easy?) and by discretization of input (not sure how to do this part)!

% Can we get bounds for MDP?


==> sections/notation.tex <==
%\subsection{Notation}

We denote by $\mathbb{R}_{\geq0}$ the non-negative reals, $\mathbb{N}$ the natural numbers and $[N]$ the set $\{0,1,\dots,N\},N\in\mathbb{N}$. Let $\mathcal{X}, \mathcal{A}\subseteq\mathbb{R}^n$. The set indicator function of $\mathcal{A}$ is $\mathbb{1}_{\mathcal{A}}(x)$, where $\mathbb{1}_{\mathcal{A}}(x)=1$ if $x\in {\mathcal{A}}$ and $\mathbb{1}_{\mathcal{A}}(x)=0$ otherwise. The set-wise difference is $\mathcal{A}\setminus \mathcal{X} = \{x\in \mathcal{A}: x\notin  \mathcal{X}\}$; the complement of a $\mathcal{A}$ is denoted as $\mathcal{A}^c$. Further, $\land$ and $\lor$ denote the logical conjunction and disjunction, respectively. For a sequence $x_{0:N}$, we use $x_{0:N}\in \mathcal{A}$ to denote $x_k\in \mathcal{A},\: \forall \:k\in [N]$. 

==> sections/preliminaries.tex <==
% \section{Preliminaries}
% \label{sec_prelim}






\subsection{Dynamic Programming}
\label{sec_dyn_prog}
For a given policy $\pi\!\in\!\Pi$ and initial state $x_0\!\in\!\mathcal{X}$, the cost incurred over $N$ time steps is
$
    C_0^{\pi}(x_0)\!=\!\mathbb{E}_{x_{0}}^\pi\!\left[ \ell_N(x_N)\!+\!\sum_{k=0}^{N-1}\! \ell_k(x_k,\mu_k(x_k)) \right]
    \label{eq_min_DP_cost_problem}
$.
The cost can be recursively computed using the DP recursion \cite{bertsekas2012dynamic}
\begin{equation}\label{cost_DP}
\begin{aligned}
    \begin{split}
        C_N^{\pi}(x_N)\!&=\!\ell_N(x_N), \\
        C_k^{\pi}(x_k)\!&=\hspace{-0.2em}\ell_k(x_k,u_k)\!+\hspace{-0.4em}\int_{\mathcal{X}}\hspace{-.7em}C_{k+1}^{\pi}(x_{k+1})T(dx_{k+1}|x_k,\!u_k),
         \end{split}
\end{aligned}
\end{equation}
where $u_k\sim\mu_k(x_k)$.
The finite-horizon optimal control problem now aims to find the infimum expected cost over the policies $\pi\in\Pi$. Denoting $C_k^{\star}(x_k):=\inf_{\pi \in \Pi}C_k^{\pi}(x_k)$, we obtain \cite{bertsekas2012dynamic}
\begin{align}\label{eq_max_cost_evaluation}
    \begin{split}
        C_N^{\star}(x_N)\!&=\!\ell_N(x_N), \\
         C_k^{\star}(x_k)\!&=\hspace{-0.4em}\min_{u_k\in\mathcal{U}}\hspace{-0.2em}\ell(x_k,u_k)\!+\hspace{-0.4em}\int_{\mathcal{X}}\hspace{-0.6em}C_{k+1}^{\star}(x_{k+1})T(dx_{k+1}|x_k,u_k).
    \end{split}
\end{align}
The minimum is attained under Assumption \ref{assumption_of_attainability} \cite{ioffe2005generic}. The optimal deterministic Markov policy described by the DP recursion \eqref{eq_max_cost_evaluation} is also optimal within the class of mixed policies \cite[Theorem 3.2.1]{hernandez2012discrete}.


\subsection{Safety}
Success in safety tasks can be captured through products of set indicator functions as
\begin{align*}
\begin{split}
    \prod_{k=0}^N\mathbb{1}_{\mathcal{A}}(x_k)&=\begin{cases}
        1 & \text{if $x_{0:N}\in\mathcal{H}_\text{I}$}, \\
        0 & \text{otherwise},
    \end{cases} \\
     1-\prod_{k=0}^N(\mathbb{1}_{\mathcal{T}^c}(x_k))&=\begin{cases}
        1 & \text{if $x_{0:N}\in\mathcal{H}_\text{R}$}, \\
        0 & \text{otherwise},
    \end{cases} \\
    1-\prod_{k=0}^N\left(1-\mathbb{1}_{\mathcal{T}}(x_k)\prod_{i=0}^{k-1}\mathbb{1}_{\mathcal{A}}(x_i) \right)&=\begin{cases}
        1 & \text{if $x_{0:N}\in\mathcal{H}_{\text{RA}}$}, \\
        0 & \text{otherwise}.
    \end{cases} 
\end{split}
%\label{eq_secSpecs_based_on_prod_of_indicator}
\end{align*}
The probability of success is then given as the expected value of the above terms; for instance, for invariance
$
    \mathbb{P}_{x_0}^{\pi}(x_{0:N}\in\mathcal{H}_{\text{I}}) = \mathbb{E}_{x_0}^{\pi}\left[\prod_{k=0}^N\mathbb{1}_{\mathcal{A}}(x_k)\right].
$
This quantity can be computed via a DP recursion with multiplicative cost, by recursively evaluating the product. We use $V_k^{\pi},V_k^{\star}:\mathcal{X}\rightarrow[0,1]$ as shorthand notation for $V_k^{\pi}(x_k)=\mathbb{P}_{x_0}^{\pi}(x_{k:N}\in \mathcal{A}|x_k, \pi)$ and $V_k^{\star}(x_k)=\sup_{\pi\in\Pi_{\text{mix}}} \mathbb{P}_{x_0}^{\pi}(x_{k:N}\in \mathcal{A}|x_k, \pi)$, respectively. Following  \cite{abate2008probabilistic}, for a given $\pi\in\Pi$ 
\begin{align}
    \begin{split}
        V_N^{\pi}(x_N) & =\mathbb{1}_{\mathcal{A}}(x_N), \\
        V_k^{\pi}(x_k) &= \mathbb{1}_{\mathcal{A}}(x_k)\hspace{-0.4em}\int_{\mathcal{X}}\hspace{-0.6em}V_{k+1}^\pi(x_{k+1})T(dx_{k+1}|x_{k}, u_k),
         \end{split}
    \label{eq_invariance_evaluation}
\end{align}
where $u_k\sim\mu_k(x_k)$, and
\begin{align}
    \begin{split}
        V_N^{\star}(x_N)\!&=\mathbb{1}_{\mathcal{A}}(x_N),\\
        V_k^{\star}(x_k)\!&=\!\max_{u_k\in\mathcal{U}}\hspace{-0.2em}\mathbb{1}_\mathcal{A}(x_k)\hspace{-0.4em}\int_{\mathcal{X}}\hspace{-0.6em}V_{k+1}^{\star}(x_{k+1})T(dx_{k+1}|x_{k}, u_k).
    \end{split}
    \label{eq_max_invariance_evaluation}
\end{align}
where the maximum is guaranteed to be attained by Assumption \ref{assumption_of_attainability} \cite{kariotoglou2017linear}. Similar recursions can be constructed to compute reachability and reach-avoid probabilities, see \cite{kariotoglou2017linear,schmid2022probabilistic}.

The existence of a feasible finite cost policy in Assumption \ref{assumption_of_attainability} can be verified by computing the safest policy, verifying that its safety is greater than $\alpha$ and its cost is finite via recursion \eqref{cost_DP}. 



==> sections/problem_statement.tex <==
\section{Preliminaries and Problem Formulation}
\label{sec_problem}
We define a Markov Decision Process (MDP) over a finite time horizon as a tuple $(\mathcal{X}, \mathcal{U}, T, \ell_{0:N})$, where the state space $\mathcal{X}$ and the input space $\mathcal{U}$ are Borel subsets of complete separable metric spaces equipped with the respective $\sigma$-algebras $\mathcal{B}(\mathcal{X})$ and $\mathcal{B}(\mathcal{U})$. Given a state $x_k\!\in\!\mathcal{X}$ and an input $u_k\!\in\!\mathcal{U}$, the stochastic kernel $T\!:\!\mathcal{B}(\mathcal{X})\!\times\!\mathcal{X}\!\times\!\mathcal{U}\!\rightarrow\![0,1]$ describes the stochastic state evolution, leading to $x_{k+1}\sim T(\cdot|x_k,u_k)$.
Additionally, $\ell_k\!:\!\mathcal{X}\!\times\mathcal{U}\!\rightarrow\!\mathbb{R}_{\geq 0}, k\in[N-1]$ and $\ell_N\!:\!\mathcal{X}\!\rightarrow\!\mathbb{R}_{\geq 0}$ denote measurable, non-negative functions called stage and terminal costs, respectively, which are incurred at every time step $k\in[N-1]$ and at terminal time $N\in\mathbb{N}$. 

%For $k \in[N-1]$ we define the space of histories up to time $k$ recursively as $\mathcal{H}_k = \mathcal{X}\times\mathcal{U} \times \mathcal{H}_{k-1}$, with $\mathcal{H}_0 = \mathcal{X}$; a generic element $h_k \in {\mathcal{H}_k}$ is of the form $h_k = (x_0, u_0, x_1, u_1, \ldots, x_{k-1}, u_{k-1}, x_k)$. We consider the following classes of policies:
 
%A stochastic policy is a sequence $\pi=(\mu_0,\dots,\mu_{N-1})$ of Borel-measurable stochastic kernels $\mu_k, k\in[N-1]$, that, given $h_k$, assigns a probability measure $\mu_k(\cdot,h_k)$ on the set $\mathcal{B}(\mathcal{U})$. 
A deterministic Markov policy is a sequence $\pi=(\mu_0,\mydots,\mu_{N-1})$ of measurable maps $\mu_k\!:\!\mathcal{X}\!\rightarrow\!\mathcal{U}, k\in [N-1]$. 
%A policy is further called Markov if $\mu_k(\cdot | h_k) = \mu_k(\cdot | x_k)$ for all $h_k\in \mathcal{H}_k$ and $k\in[N-1]$. Otherwise, it is called causal. 
We denote the set of deterministic Markov policies by $\Pi$. In this work, we define mixed policies $\pi_{\text{mix}}$ as a deterministic Markov policy that is randomly chosen at the initial time step $k=0$ and then used during the entire control task. More formally, we endow the set $\Pi$ with the metric topology and define the corresponding Borel $\sigma$-algebra by $\mathcal{G}_{\Pi}$ \cite{aumann_1}. A mixed policy $\pi_{\text{mix}}$ can be seen as a random variable on the measurable space $(\Pi,\mathcal{G}_{\Pi})$. The set of all mixed policies is denoted as $\Pi_{\text{mix}}$. Note that $\Pi\subseteq\Pi_{\text{mix}}$.

For a given initial state $x_0\in\mathcal{X}$, policy $\pi\in\Pi$, and transition kernel $T$, a unique probability measure $\mathbb{P}_{x_0}^{\pi}$ for the state-input-trajectory is defined over $\mathcal{B}((\mathcal{X} \times \mathcal{U})^N\times \mathcal{X})$, which can be sampled recursively via $x_{k+1}\sim T(\cdot|x_k,\mu_k(x_k))$ \cite{abate2008probabilistic}. We define the associated expected cumulative cost as  
%{\color{red} I would reverse the order, i.e., first sum over stage cost and then terminal set..just to be in line with $(\mathcal{X} \times \mathcal{U})^N\times \mathcal{X}$..very minor stuff}
\begin{align*}
    &\mathbb{E}_{x_0}^\pi 
\left[ \ell_N(x_N) + \sum_{k=0}^{N-1} \ell_k(x_k,u_k) \right]=\hspace{-.4cm}\int\displaylimits_{(\mathcal{X} \times \mathcal{U})^N\times \mathcal{X}}\hspace{-.6cm}\biggl(\ell_N(x_N)\! \\ &\qquad+\!\sum_{k=0}^{N-1} \ell_k(x_k,u_k)\!\biggl)\mathbb{P}_{x_0}^{\pi}(dx_0,du_0,\dots,dx_N).
\end{align*}
%Since the probability measure over trajectories $\mathbb{P}_{x_0}^{\pi}$ associated to any policy $\pi$ and starting from the initial state $x_0$ is unique, the associated expected cost is unique. 
Since the probability measure over trajectories $\mathbb{P}_{x_0}^{\pi}$ is unique, it follows that the expected cost is also unique.  %Interestingly, for any stochastic causal policy, the most general realizable policy class, there exists a mixed policy that yields exactly the same probability measure $\mathbb{P}_{x_0}^{\pi}$ and hence the same cost \cite{schmid2023Jccoc}. Consequently, we consider solving the upcoming problems over the class of mixed policies, yielding the best achievable performance.

\subsection{Problem Formulation}
\label{sec_problem_formulation}
In addition to minimizing cost we aim to synthesize controllers that meet additional specifications. Let $\mathcal{A},\mathcal{T}\in\mathcal{B}(\mathcal{X})$ define a safe set and target set, respectively, such that $\mathcal{A}\cap\mathcal{T}=\varnothing$. The set of trajectories satisfying specifications called invariance, reachability, and reach-avoidance, are defined respectively as
\begin{align*}
    \mathcal{H}_{\text{I}}\!&=\! \{x_{0:N}\in\mathcal{X}^{N+1}\!:\!x_{0:N}\in\mathcal{A}\}, \\
    \mathcal{H}_{\text{R}}\!&=\! \{x_{0:N}\in\mathcal{X}^{N+1}\!:\!\exists x_k\in x_{0:N}, x_k\in\mathcal{T}\}, \\
    \mathcal{H}_{\text{RA}}\!&=\! \{x_{0:N}\in\mathcal{X}^{N+1}\!:\!\exists x_k\in x_{0:N}, x_{0:{k-1}}\in\mathcal{A} \land x_k\in\mathcal{T}\}. 
\end{align*}


Let $\mathcal{H}\in\{\mathcal{H}_{\text{I}},\mathcal{H}_{\text{R}},\mathcal{H}_{\text{RA}}\}$. Our aim is to minimize the cumulative cost, while guaranteeing a prescribed probability of satisfying the specification $\mathcal{H}$, leading to the joint chance constrained optimal control problem
\begin{equation}\label{eq_problemFormulation_CCOC}
\begin{aligned} 
    \begin{split}
    \inf_{\pi \in \Pi_{\text{mix}}} \quad  &\mathbb{E}_{x_0}^\pi\left[ \ell_N(x_N) + \sum_{k=0}^{N-1} \ell_k(x_k,u_k) \right]\\
    \text{s.t.} \quad  & \mathbb{P}_{x_0}^\pi(x_{0:N}\in \mathcal{H})\geq \alpha,
    \end{split}
\end{aligned}
\end{equation}
where $\alpha \in [0,1]$ is a user-specified success probability. 
%We restrict to finding solutions in the space of mixed deterministic Markov policies. However, this is without loss of generality. Generally one would aim to solve Problem \eqref{eq_problemFormulation_CCOC} over the class of stochastic causal policies, which is the most general policy class. However, as shown in \cite{schmid2023Jccoc}, it is sufficient to consider solutions of Problem \eqref{eq_problemFormulation_CCOC} within the space of mixed deterministic Markov policies without sacrificing optimality. 
As shown in \cite{schmid2023Jccoc}, the restriction in Problem \eqref{eq_problemFormulation_CCOC} to the class of mixed policies is without loss of optimality when compared to the class of stochastic causal policies.
For simplicity, we term the probability of satisfying the additional specification as safety probability, irrespective of the type of objective, and call a trajectory safe if $x_{0:N}\in\mathcal{H}$.

To ensure the existence of an optimal policy in Problem \eqref{eq_problemFormulation_CCOC}, we introduce the following standing assumption.
\begin{assumption}\label{assumption_of_attainability}
    The input set $\mathcal{U}$ is compact. For all $x\in\mathcal{X}$, $\mathcal{C}\in\mathcal{B}(\mathcal{X})$, the transition kernel $T(\mathcal{C}|x,u)$ and stage cost $\ell_k(x,u)$ are continuous with respect to $u$. A feasible finite cost policy for Problem \eqref{eq_problemFormulation_CCOC} exists.
\end{assumption}
To simplify the notation we further assume that the stochastic kernel $T$ admits a density $t$. However, all of our results extend to kernels that admit no density. They also extend to finite state and action spaces. %Further, all of our results extend to finite state and action spaces.
%As shown later, if Problem \eqref{eq_problemFormulation_CCOC} is feasible, the infimum is attained under Assumption \ref{assumption_of_attainability}. Note that, to streamline the presentation, we rely on assumptions that are more restrictive than necessary; alternative sufficient conditions can be found in \cite{hernandez2012discrete}.



% In this work, we aim to solve Problem \eqref{eq_problemFormulation_CCOC} using its Lagrange-Dual
% \begin{equation}\label{eq_dual_of_CCOC}
%     \begin{split}
%         \max_{\lambda\in\mathbb{R}_{\geq 0}}\inf_{\pi \in \Pi} \quad  &\mathbb{E}_{x_0}^\pi\left[ \ell_N(x_N) + \sum_{k=0}^{N-1} \ell_k(x_k,u_k) \right] \\ &+ \lambda(\alpha-\mathbb{P}_{x_0}^\pi(x_{0:N}\in \mathcal{H})).
%     \end{split}
% \end{equation}
% However, the inner minimization is intractable due to the non-Markovian structure imposed by the constraint (see \cite{schmid2023Jccoc}). In what follows, we will formulate DP and LP based methods that alleviate the intractability of the problem and provide provably optimal solutions. 


%Finally, let the set $\mathcal{A} \subseteq \mathcal{B}(\mathcal{X})$ denote a safe set.  
% \\ \intertext{and the probability of safety as} 
%     &\mathbb{P}_{x_0}^\pi(x_{0:N}\in \mathcal{A})=\hspace{-.7cm}\int\displaylimits_{(\mathcal{X} \times \mathcal{U})^N\times \mathcal{X}}\!\prod_{k=0}^{N-1}\! \mathbb{1}_{\mathcal{A}}(x_k)\mathbb{P}_{x_0}^{\pi}(dx_0,du_0,\dots,dx_N),

==> sectionsRev1/ApproximationsForContSpaces.tex <==


\section{Approximations for Continuous Spaces}
\label{sec_approx_for_cont}
Recall that the constraints in LP \eqref{eq_lp_ccoc} must hold over all states and inputs; infinitely many if the state and input spaces are continuous. In such cases approximations have to be introduced, e.g., via gridding or basis functions. Therefore, in the following we impose the state space $\Tilde{\mathcal{X}}$ to be compact.

\subsection{Gridding}
Let there be a finite partitioning of the state and input space into $\Tilde{\mathcal{X}} = \cup_{j=1}^{M_x}\Tilde{\mathcal{X}}_j$ and $\mathcal{U}=\cup_{j=1}^{M_u}\mathcal{U}_j$, where each set $\Tilde{\mathcal{X}}_j$ has non-zero $\nu$-measure, $M_x, M_u \in\mathbb{N}$. The sets $\Tilde{\mathcal{X}}_j$ are chosen such that they do not contain states with differing values for the augmented states and the MDP state components are fully contained in either $\mathcal{A},\mathcal{T}$ or $\mathcal{X}\setminus(\mathcal{A}\cup \mathcal{T})$. Let $\{\Tilde{s}_j\in\Tilde{\mathcal{X}}_j\}_{j=1}^{M_x}$ and $\{a_j\in\mathcal{U}_j\}_{j=1}^{M_u}$ be arbitrary points of these sets and the grid size of the discretization be defined as $\Delta = \max_{1\leq j \leq M_x}\sup_{\Tilde{x}_1,\Tilde{x}_2\in \Tilde{\mathcal{X}}_j}||\text{proj}_{\mathcal{X}}(\Tilde{x}_1-\Tilde{x}_2)||_2$, where $\text{proj}_{\mathcal{X}}(\cdot)$ denotes the projection onto the space $\mathcal{X}$. %and $\delta_u = \max_{1\leq j \leq M_u}\sup_{u_1,u_2\in \mathcal{U}_j}||x_1-x_2||_2$. 
For the resulting finite MDP the LP \eqref{eq_lp_ccoc} reads as
\begin{equation}
    \begin{split}
        \max_{\substack{ \lambda\in\mathbb{R}_{\geq 0},\\J_{0:N}\in \mathbb{R}^{M_x} }} \quad  &J_{0,l}
        \\ \text{s.t.} \quad &J_{N,j}\leq\ell_N(\Tilde{s}_j)  +\lambda(\alpha-\delta(b_j)), \\
        &J_{k,j}\leq  \ell_k(\Tilde{s}_j,a_i) +\hspace{-1em} \sum_{1\leq j' \leq M_x}\hspace{-1em}J_{k+1,j'}\Tilde{T}(\Tilde{X}_{j'}|\Tilde{s}_j,a_i),
    \end{split}
    \label{eq_lp_ccoc_discrete}
\end{equation}
where $b_j$ is the augmented state of $\Tilde{s}_j$, $l\in[0,M_x]$ is the index of the set $\Tilde{\mathcal{X}}_l$, which contains the initial state $\Tilde{x}_0$, $J_{k,j}$ denotes the $j$'th entry of the vector $J_k$ and the constraints hold for all $1\leq j \leq M_x$, $1\leq i \leq M_u$. The discrete version of the LP \eqref{eq_lp_ccoc_value_functions} follows accordingly. The optimal mixed policy for the discretized version of Problem \eqref{eq_problemFormulation_CCOC} is constructed by mixing the cheapest and safest greedy policies on the resulting value functions. %The set of optimal inputs at a given state and time step is easily identified by the set of active constraints of the LP \eqref{eq_lp_ccoc_discrete}. 
Under the mixing ratios in \eqref{eq_stochastic_policies_ratios}, the mixed policy yields a safety of $\alpha$ when applied to the discretized dynamics. However, when applied to the continuous dynamics, the safety of the policy potentially deteriorates. Furthermore, the extent of deterioration is computationally hard to determine. Instead, we provide bounds on the difference of safety between the discretized and continuous dynamics in the following. When faced with continuous dynamics, the policy obtained for the discretized dynamics is implemented such that, if the continuous state $\Tilde{x}_k\in \Tilde{\mathcal{X}}_j, 1\leq j \leq M_x$, the action advertised for the state $\Tilde{s}_j$ is applied to the system. 
% \begin{assumption}
%     \begin{align*}
%         |t(x_{k+1}|x_k,u_k) - t(x_{k+1}|x_k,u_k')|\leq h_u||u-u'|| 
%     \end{align*} for all $x_{k+1},x_k\in\mathcal{X}, u_k,u_k'\in \mathcal{U}$.
% \end{assumption}
% \begin{proposition}
%     Let the MDP be finite, $\hat{J}_{0:N}^{\text{LP}}$ be the optimal solution of \eqref{eq_lp_ccoc_value_functions} under the optimal $\lambda$ in \eqref{eq_lp_ccoc}. Let  $\hat{J}_{0:N}^{\star}$ be the value functions associated to the optimal policy of Problem \eqref{eq_dual_of_CCOC}. Then, $\hat{J}_{0:N}^{\text{LP}}=\hat{J}_{0:N}^{\star}$. Further, the greedy policy on $\hat{J}_{0:N}^{\text{LP}}$ coincides with the state-input pairs that form active constraints in the LP \eqref{eq_lp_ccoc_value_functions}.
% \end{proposition}
% \begin{proof}
%     The equivalence of $\hat{J}_{0:N}^{\text{LP}}=\hat{J}_{0:N}^{\star}$ is a direct consequence of tdoref, since any representative point $x_j$ is associated non-zero $v$-measure.

    
% \end{proof}
% Above Proposition is useful in two ways. Firstly, it allows to characterize the optimal policies by the active constraints of the LP. Using the recursions tdoref and tdoref and restricting to inputs that form active constraints at the given state, we can solve for the cheapest and safest $\lambda^{\star}$-optimal policies $\pi_c$ and $\pi_v$. Note that the analysis in \cite{schmid2023Jccoc}, which holds for finite as well as continuous systems. Hence, if Problem \eqref{eq_problemFormulation_CCOC} is feasible for the discretized dynamics, the policy $\pi_v$ will have a safety of at least $\alpha$. Let the associated safety and costs in the discretized formulation, computed using recurions tdoref and tdoref, be $\hat{V}_{\pi_c}$, $\hat{V}_{\pi_v}$, $\hat{C}_{\pi_c}$ and $\hat{C}_{\pi_v}$, respectively. Let the policies be mixed according to 
% \begin{align}
% \label{eq_stochastic_policies_ratios}
% \pi_{\text{mix}}=\begin{cases}
% \pi_{\overline{\lambda}} & \text{with probability } p_{\overline{\lambda}}\!=\!\frac{\alpha - V_0^{\pi_{\underline{\lambda}}}(\Tilde{x}_0)}{V_0^{\pi_{\overline{\lambda}}}(\Tilde{x}_0) - V_0^{\pi_{\underline{\lambda}}}(\Tilde{x}_0)}, \\
% \pi_{\underline{\lambda}} & \, \text{otherwise.}
% \end{cases}
% \end{align}
% Then, under the discretized dynamics, the mixed policy solves Problem \eqref{eq_problemFormulation_CCOC} to optimality \cite{schmid2023Jccoc}. 


%This is easily obtained from the safety of its constructing policies which has been computed via recursion tdoref to solve for the optimal mixing probabilities. Let the safety of the mixed policy, when applied to the continuous system, be denoted by $V_{\pi_{\text{mix}}}$, which is usually hard to compute in practice. 
\begin{assumption}
    The transition kernel $T$ admits a Lipschitz continuous density $t$, \begin{align*}
        |t(x_{k+1}|x_k,u_k) - t(x_{k+1}|x_k',u_k)|\leq h_x||x_k-x_k'||, 
    \end{align*} for all $x_{k+1},x_k,x_k'\in\mathcal{X}, u_k\in \mathcal{U}$.
    \label{ass_lipschitz_cont}
\end{assumption}
\begin{proposition}
    Let the safety of the mixed policy $\pi_{\text{mix}}$ at the initial state $x_0$ when applied to the continuous dynamics be denoted by $\hat{v}_{\pi_{\text{mix}}}$, and when applied to the discretized dynamics be denoted by $v_{\pi_{\text{mix}}}$. Under Assumption \ref{ass_lipschitz_cont}, the safety of $\pi_{\text{mix}}$ applied to the continuous system is bounded by $||\hat{v}_{\pi_{\text{mix}}}-v_{\pi_{\text{mix}}}||\leq N\gamma h_x\Delta$, where $\gamma$ is the Lebesgue measure of the set $\mathcal{A}$ for invariance and reach-avoid specifications and $\mathcal{X}\setminus\mathcal{T}$ for reachability specifications.
\end{proposition}
\begin{proof}
    Let the safety of the cheapest and safest $\lambda^{\star}$-optimal policy when evaluated on the discretized dynamics by denoted by $v_{c}$ and $v_{v}$, and when applied to the continuous system be denoted by $\hat{v}_{c},\hat{v}_{v}$, respectively. We know that $||\hat{v}_{c}-v_{c}||\leq N\gamma h_x\Delta$ and $||\hat{v}_{v}-v_{v}||\leq N\gamma h_x\Delta$ by \cite{abate2010approximate}. Hence, for any mixed policy, which has safeties $p_{v}v_{v} + (1-p_{v})v_{c}$ when evaluated on the discretized dynamics and $p_{v}\hat{v}_{v} + (1-p_{v})\hat{v}_{c}$ when applied to the continuous dynamics, respectively, we obtain 
    \begin{align*}
        ||\hat{v}_{\text{mix}}\!-\!v_{\text{mix}}||\!
        &=\!||p_{v}\hat{v}_{v}\!+\!(1\!-\!p_{v})\hat{v}_{c}\!-\!p_{v}v_{v}\!-\!(1\!-\!p_{v})v_{c}||\\
        &\leq\!||p_{v}(\hat{v}_{v}\!-\!v_{v})||\!+\!||(1\!-\!p_{v})(\hat{v}_{c}\!-\!v_{c})||\\
        &\leq\!|p_{v}|N\gamma h_x\Delta\!+\!|(1\!-\!p_{v})|N\gamma h_x\Delta\\
        &=\!N\gamma h_x\Delta.
    \end{align*}
\end{proof}
Since this bound can be computed a-priori, the safety level $\alpha$ can be tightened accordingly to guarantee a desired safety probability despite errors introduced by gridding.



% \begin{proposition}
%     Let $\lambda^{\star}$ be zero. Taking the safest $\lambda^{\star}$-optimal policy is an optimal solution. Let $\lambda^{\star}$ be equal to one, then the cheapest $\lambda^{\star}$-optimal policy is the optimal solution if it has safety greater $\alpha$. If not, the problem is infeasible. Let $\lambda^{\star}\in(0,1)$. The mixed policy tdoref is the optimal solution to the discrete LP.
% \end{proposition}
% \begin{proof}
%     First two cases are trivial. Third case:
%     The space of lambda optimal policies forms a single point or a continuous line (since it is convex) in the performance set. Taking the cheapest and the safest policy among the lambda optimal policies we can obtain the performances of all policies on the line by interpolation. Since $\lambda^{\star}$ is optimal, the optimal mixed policy is on that line and has safety $\alpha$. Hence, we can construct it by interpolating as in eq. tdoref.
% \end{proof}
%and $\pi_c$ and $\pi_v$ the associated minimum cost and maximum secondary policy. 

\subsection{Basis Function Approximations}
An alternative approach lies in approximating the value functions using basis functions, i.e., $J_{k}(\Tilde{x}_k)=\sum_{i=0}^{M-1}\beta_i\phi_i(\Tilde{x}_k)$, with parameters $\beta_i\in\mathbb{R},i\in[M-1]$ and basis functions $\phi_i:\Tilde{\mathcal{X}}\rightarrow\mathbb{R}$ \cite{defarias2003linear, mohajerin2018infinite, schmid2022probabilistic}. The $M$ basis functions are chosen a-priori and the LP optimizes over the parameters $\beta_i$. Due to approximation errors and computational aspects, it is not meaningful to compute the safest and cheapest greedy policies on the value functions obtained by LP \eqref{eq_lp_ccoc_value_functions}. Instead, one might directly apply any greedy policy associated to the results of LP \eqref{eq_lp_ccoc_value_functions} under an optimal $\lambda$ of LP \eqref{eq_lp_ccoc}, yielding the method a heuristic without explicit guarantees but with potentially better scalability than gridding. 

%We further aim to solve Problem \eqref{eq_dual_of_CCOC} under basis-function approximations of the value functions $J_{k}(x_k)=\sum_{i=M}\beta_i\phi_i(x_k)$, with parameters $\beta\in\mathbb{R}$ and basis functions $\phi_i:\mathcal{X}\rightarrow\mathbb{R}$ \cite{defarias2003linear}. The $M$ basis functions are chosen a-priori and the LP optimizes over the parameters $\beta_i,i\in[M]$. Under this approximation method, it is not practically meaningful to compute the safest and cheapest policy within the $\lambda^{\star}$ optimal policies due to approximation errors incurred by this method. Instead we directly apply the greedy policy associated to the results of Problem \eqref{eq_lp_ccoc_value_functions} under an optimal $\lambda$ of Problem \eqref{eq_lp_ccoc}. We do not provide conditions that guarantee optimality of the method, leaving basis function approximations as a useful heuristic without guarantees. We analyse the performance of the approach numerically instead.

==> sectionsRev1/acronym.tex <==
\begin{acronym}
\acro{ADP}{Approximate Dynamic Programming}
\acroindefinite{ADP}{an}{a}

\acro{BSA}{Basic Semialgebraic}

\acro{LP}{Linear Program}
\acroindefinite{LP}{an}{a}
\end{acronym}

==> sectionsRev1/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
\IEEEPARstart{M}{ost} system dynamics are non-deterministic, either naturally or due to unobservable modes, e.g., variability of large scale processes \cite{pitchford2007uncertainty, fochesato2022data} or robotic path planning in uncertain environments \cite{schmid2022real, blackmore2011chance}. While control problems often feature a ``real" control cost objective, e.g., energy consumption or negative financial profit, additional objectives often need to be included, such as reaching or remaining in a set of states, e.g., for safety. Such behaviours can be imposed in optimal control problems by manually shaping the cost associated to individual states until the policy behaves as desired. However, without any instructive procedure it is generally hard to achieve clear trade-offs between safety guarantees and the control cost \cite{Ono_2}. %The control-engineer needs a clear method to trade off safety vs. cost without requiring deep expertise or extensive finetuning of parameters.

The task of remaining in a safe set is called \textit{invariance}, that of reaching a target set \textit{reachability}, while \textit{reach-avoidance} combines both objectives. The goal of finding a policy that yields an optimal trade-off between the control cost incurred by the system and the probability of achieving one of the above specifications is described by the so called joint-chance constrained optimal control problem (cf. \cite{schmid2023Jccoc}). While this class of problems is very popular, existing solution approaches are computationally challenging due to the non-Markovian structure imposed by these constraints (cf. \cite{Wang}). To overcome these computational issues, the state-of-the-art is to utilize approximations based on conservative bounds \cite{Ono_2, paulson, patil_1, wang2020non, nemirovski2007convex, hokayem2013chance, blackmore2011chance} or approximate the stochastic elements via sampling \cite{thorpe_1
%, raghuraman
, huang2021risk}. 


A recently evolving idea is to break the non-Markovian structure using a state-augmentation, resulting in a conventional Markov Decision Process (MDP) \cite{schmid2023Jccoc, haesaert2021formal, hahn2019interval}. In \cite{hahn2019interval}, a value iteration algorithm is formulated to solve the full Pareto front for interval MPDs with multiple probabilistic temporal logic objectives. In \cite{haesaert2021formal}, a linear program (LP) on occupation measures for interval MPDs is formulated to find trade-offs between multiple probabilistic temporal logic objectives. However, the proposed solutions feature only interval MDPs with finite states and actions and the potential suboptimality of the computed policies remains unaddressed. In \cite{schmid2023Jccoc}, the joint chance constrained problem is approached via a bilevel optimization on its Lagrange dual, requiring to iteratively solve Dynamic Programming (DP) recursions. A suboptimality bound to the global optimum is presented, which decreases exponentially with the number of DP iterations. %Hence, the solution is proven to converge to a globally optimal policy and there is no duality gap. 
Unfortunately, the suboptimality bound in \cite{schmid2023Jccoc} convergences to an optimal policy only in the limit, while it is desirable to obtain a provably optimal policy in finitely many computations. This paper closes this gap. 

\textbf{Contribution.} As our main contribution we show that the bilevel problem in \cite{schmid2023Jccoc} can be solved via a sequence of two LPs. We prove that the obtained policy is an optimal solution to the joint chance constrained optimal control problem. To extend the applicability of our results we provide instructions on how to extend the safety specification in \cite{schmid2023Jccoc} from invariance to reach-avoid specifications. Faced with large or continuous state spaces, the LP framework allows for basis function approximations with generally superior scalability compared to gridding~\cite{de2003linear}.%, although, we do not explore this fact in detail for the sake of brevity.   


% If the state- and actions spaces are continuous, the approach in \cite{schmid2023Jccoc} is restricted to gridding based approximations. The linear programming based approaches further allow for more general function approximations 
% 

% Recently, \cite{schmid2023Jccoc} proposed a novel, numerically tractable Dynamic Programming (DP) algorithm that allows to determine optimal trade-offs between control cost and invariance probabilities. Moreover, the suboptimality of the solution decreases exponentially with the number of algorithm iterations. In this paper we extend this framework in the following directions: 
% \begin{itemize}
%     \item we include reachability and reach-avoid specifications;
%     \item we compute policies using a one-shot linear programming (LP) approach with no residual suboptimality.
% \end{itemize}



%    \item we provide error bounds for the optimal policy when continuous state and action spaces are discretized. 
%an instructive discussion to manage problems with continuous state and action spaces, where approximations are required. We present error bounds under gridding. Further, as a useful heuristic, our linear programming formulation allows the use of basis function approximations (approximate dynamic programming), which provides a superior scalability with the dimensionality of the state and action space over gridding. 

%It is the aim of this paper to design in particular such algorithms, that can optimally trade off the probability of satisfying a reachability, invariance, or reach-avoid specification, against increase of costs. 

%Section \ref{sec_problem} formally introduces the joint chance constrained optimal control problem. Section \ref{sec_prelim} introduces tools used by current DP-based approaches (Section \ref{sec_jcc_dp}) and our LP-based approach (Section \ref{sec_jcc_lp}) to solve such types of problems. Approximations for systems with continuous state and action spaces are discussed in Section \ref{sec_approx_for_cont} and numerically  evaluated in Section \ref{sec_examples}. We conclude with Section \ref{sec:conclusion}.

